A Robust Algorithm for Tile-based 360-degree Video Streaming with Uncertain FoV Estimation

We propose a robust scheme for streaming 360-degree immersive videos to maximize the quality of experience (QoE). Our streaming approach introduces a holistic analytical framework built upon the formal method of stochastic optimization. We propose a robust algorithm which provides a streaming rate such that the video quality degrades below that rate with very low probability even in presence of uncertain head movement, and bandwidth. It assumes the knowledge of the viewing probability of different portions (tiles) of a panoramic scene. Such probabilities can be easily derived from crowdsourced measurements performed by 360 video content providers. We then propose efficient methods to solve the problem at runtime while achieving a bounded optimality gap (in terms of the QoE). We implemented our proposed approaches using emulation. Using real users' head movement traces and real cellular bandwidth traces, we show that our algorithms significantly outperform the baseline algorithms by at least in $30\%$ in the QoE metric. Our algorithm gives a streaming rate which is $50\%$ higher compared to the baseline algorithms when the prediction error is high.

==> algo_mobicom.tex <==
\section{Algorithms and Results}\label{sec:result}
The problem in $\mathcal{P}_{\mathrm{eq}}$ is not a convex problem. In order to make it convex, we first relax the discrete strategy space. Subsequently, we state an algorithm (\textbf{360-ROBUST}) which computes a feasible solution from the optimal solution from the relaxed problem. Finally, we state the online version of the algorithm 360-ROBUST which adapts to the real time variation of the bandwidth prediction, and the FoV prediction. 
\subsection{Relaxation}
 %we make the following assumption.

%First, we assume that
%\vspace{-.1in}

%\feng{[[But I think Assumption 1 applies to the original problems $\mathcal{P}$ and  $\mathcal{P}_{\mathrm{eq}}$ as well, right? Move it earlier when you are describing $U(\cdot)$.]]}



%\feng{[[The description of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ is the same as $\mathcal{P}_{\mathrm{eq}}$. Make sure you highlight that $\gamma_k$ is now continuous.]]}

The relaxed problem is stated in the following:
\begin{eqnarray}
\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}: & \text{ maximize } (\ref{eq:robust})\nonumber\\%\text {maximize } &\sum_{k=1}^{K}U(\gamma_k)-\lambda(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})\nonumber\\
& \text{subject to } &  (\ref{eq:equi}), (\ref{eq:downtime}), (\ref{eq:max_buffer}),  R_{0}\leq \gamma_k\leq R_m\nonumber\\
%& & \gamma_k\leq R_{j,k} \forall j\in \mathcal{A}_{\alpha}\label{eq:robust_constraint}\\
& \text{var}: & \gamma_k\nonumber
\end{eqnarray}
Note that $\gamma_k$ is now continuous an can take any value within the interval $[R_{0},R_m]$ unlike the discrete values in 
$\mathcal{P}_{\mathrm{eq}}$. 

\begin{proposition}\label{prop:convexrobust}
$\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$  is a convex optimization problem.

The optimal value of the objective function in $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$  is greater than or equal to the optimal value of the objective function in $\mathcal{P}_{\mathrm{eq}}$. 
\end{proposition}
Since the relaxed problem $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ is convex, we can solve it using the standard convex optimization techniques efficiently. However, we have to transform the optimal solution of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ into a feasible solution as the optimal solution $R^{*}_{i,k}$ of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$  may not belong to the discrete set $\{R_0, . . . , R_m\}$. Since the strategy space is relaxed, the optimal value will be greater than or equal to the optimal value of the exact problem. The equality arises only when the solution of the relaxed problem is a feasible solution of the exact problem. In the following section, we provide a heuristic solution to obtain the feasible solutions from the optimal solution of the relaxed problem.
%\vspace{-.1in}
\subsection{Heuristic to obtain the feasible solution}
Let $\gamma^{*}_k$ be the optimal solution of the relaxed problem $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ for all $k$. $\gamma_{k}^{*}$ can be obtained using the convex optimization tools as the problem is convex (Proposition~\ref{prop:convexrobust}). Now, we describe a simple heuristic to obtain a feasible solution based on the optimal solution.
%\begin{algorithm}
\begin{figure}
	\vspace{-.1in}
\begin{algorithm}[H]
\small
\begin{algorithmic}
\STATE {\bf Inputs}: $\mathcal{A}_{\alpha,k}$, $C_k$, the optimal solution $\gamma^{*}_k$ of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$, and the set  $\{R_0,\ldots, R_m\}$.
\STATE {\bf Initialization:} $L_0=0$.
\FOR{$k=1,\ldots, K$}
%\FOR{$i=1,\ldots, N$}
\STATE $\gamma_k=\max_{j\in\{1,\ldots,m\}} \{R_{j}: R_{j}\leq \gamma^{*}_k\}$.
\STATE $\bar{\gamma}_{k}=\min_{j\in \{1,\ldots,m\}} \{R_{j}: R_{j}\geq \gamma^{*}_{k}\}$.
%\ENDFOR
\STATE Compute $L_k=L_{k-1}+(\gamma^{*}_{k}-\gamma_{k})$.
 %\STATE $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
\ENDFOR
\IF{$L_{K}<\bar{\gamma}_{k}-\gamma_k$}
\STATE Exit since it is the optimal solution.
\ENDIF
\FOR{$k=K, K-1, \ldots , 2$}
\IF{$L_k\geq\bar{\gamma}_{k}-\gamma_k$}

\STATE $L_{k-1}=L_{k}-(\bar{\gamma}_{k}-\gamma_k)$.
\STATE Update: $\gamma_k=\bar{\gamma}_{k}$ for all $i\in \mathcal{A}_{\alpha,k}$.%\sum_{i\in \mathcal{A}_{\alpha,k}}(\bar{R}_{i,k}-R_{i,k})$.
%\STATE Update $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
\ENDIF
\ENDFOR
\STATE {\bf OUTPUT} $\gamma_k$.
\end{algorithmic}
\caption{: Algorithm \textbf{360-ROBUST} provides a feasible solution of $\mathcal{P}_{\mathrm{eq}}$ from the optimal solution of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$}\label{algo2} 
\end{algorithm}
\vspace{-0.4in}
\end{figure}
%\begin{algorithmic}
% $L_0=0$\;
%\For{$k=1,\ldots, K$}{
%\For{$i=1,\ldots, N$}{
% $R_{i,k}=\max \{R_{j}: R_{j}\leq R^{*}_{i,k}\}$\;
%$\bar{R}_{i,k}=\min \{R_{j}: R_{j}\geq R^{*}_{i,k}\}$\;
%}
%Compute $L_k=L_{k-1}+(R^{*}_{i,k}-R_{i,k})$\;
%}
%\If{$L_{K}=0$} {exit, it is the optimal solution\;}
%\For{$k=1,\ldots,K$}{
%\If{$L_k-\sum_{i\in \mathcal{A}_{\alpha,k}}(\bar{R}_{i,k}-R_{i,k})>0$}{
%Update: $R_{i,k}=\bar{R}_{i,k}$ for all $i\in \mathcal{A}_{\alpha,k}$\;
%$L_{k+1}=L_{k}-\sum_{i\in \mathcal{A}_{\alpha,k}}(\bar{R}_{i,k}-R_{i,k})$\;}
%}
%%\end{algorithmic}
%\caption{Algorithm 2}\label{algo2}
%\end{algorithm}
%\textbf{Algorithm 2}:
%\begin{enumerate}
%\item $L_0=0$.
%\item For $k=1,\ldots, K$ and $i=1,\ldots, N$ do the following
%\item Set $R_{i,k}=\{R_{j}: R_{j}\leq R^{*}_{j,k}<R_{j+1}\}$,
%\item Set $\bar{R}_{i,k}=\{\min\{R_j,R_{max}\}:R_j>R_{i,k}, R_{j-1}=R_{i,k}\}$.
%\item Compute $L_k=L_{k-1}+\sum_{i}(R^{*}_{i,k}-R_{i,k})$.
%\item End For.
%\item If $L_{K}>0$, then go to the next step, otherwise exit since it is the optimal solution.
%\item For $k=1,\ldots, K$ do the following
%\begin{enumerate}
%\item If $L_{k}-\sum_{i\in \mathcal{A}_{\alpha,k}}(\bar{R}_{i,k}-R_{i,k})> 0$,
%\item Update: $R_{i,k}=\bar{R}_{i,k}$ for $i\in \mathcal{A}_{\alpha}$ and $L_{k+1}=L_{k}-\sum_{i\in \mathcal{A}%_{\alpha,k}}(\bar{R}_{i,k}-R_{i,k})$.
%\end{enumerate}
%\item End For.
%\end{enumerate}

As described in Algorithm~\textbf{360-ROBUST}, our high-level idea is to
%\feng{[[The biggest issue with the text below is that it just mechanically describes what the algorithm does, without providing much intuition. Why the residual bandwidth propagated backward instead of forward?]]}
 set $\gamma_k$ at the maximum possible rate which is less than or equal to the optimal solution $\gamma_k^{*}$ of the relaxed problem. Hence, $\gamma_k$ is obtained by simply down-quantizing the optimal rate obtained from the relaxed problem. The algorithm proceeds to compute the bandwidth saved compared to the solution of the relaxed problem because of the down-quantization ($L_k$).

%The algorithm then assigns the rates with which the tiles should be downloaded at $\bar{\gamma}_k$ as long as $L_{k}$ is non-positive starting from the last chunk. In other words, the algorithm tries to increase the rate for each chunk for the future chunks if it does not increase the stall compared to the solution of the relaxed problem.

 The algorithm saves any additional bandwidth from down-quantization to download later chunks at the immediate higher level if it does not increase the stall duration. The algorithm reserves the saved bandwidth for fetching the last chunk at the immediate higher level. If there is a still bandwidth available it will fetch the penultimate chunk at the higher level and so on. %Specifically, the algorithm fetches the chunk $K, K-1, \ldots$ at the immediate next higher level and so on until the stall time does not increase ($L_k$ remains positive).  
 
A reader may ask the question why not assigning the additional bandwidth to fetch the earlier chunk at  a higher rate rather fetching the later chunks at a higher rate. The reasons are the following. First, this will help reduce the number of switches of rate among two consecutive chunks. If we download the next immediate chunk (say, $k$)  at a higher rate, we may still have to download the chunk $k+1$ at a lower rate which will increase the quality variation between the two consecutive chunks. 
%: first, our algorithm up-quantizes the rate to the immediate next level starting from the last chunk. If the additional bandwidth is used to fetch the nearest possible chunk at a higher rate, the other chunks may be fetched a relatively lower rate because there will be no bandwidth to increase the rates of the next chunk. Hence, the number of switches of rate among two consecutive chunks is minimum if the residual bandwidth is used to fetch the chunks at the immediate higher rate starting from the last chunk. 
Second, there may be an error in estimating the bandwidth; if the estimated bandwidth is erroneous, there may not be any bandwidth to fetch the future chunks even in the lower rate, if the additional bandwidth is used up in downloading the current chunk at the immediate higher level.%We do the above for each chunk until we reach the last chunk.  Thus, the algorithm tries to fetch the higher quality tiles for chunk $k$, then proceeds to fetch higher quality ones for chunk $k+1$, and so on.  The algorithm tries to minimize any wasted bandwidth because of the down-quantization. Hence, it will achieve a higher play-back rate compared to a simple down-quantization.

%$L_{k}$, the bandwidth that is saved because of the down-quantization of the rates. Then the algorithm tries to fetch the tiles within the set $\mathcal{A}_{\alpha,k}$ at one level higher (assigning to $\bar{\gamma}_{k}$)  provided that the stall time does not increase compared to the optimal solution of the relaxed problem ($L_{k}$ is not negative).   Note that  %The FoV can be more accurately predicted for chunks in the near future. The chunks in the near future have tighter deadlines, hence, we may see low quality chunks at the beginning, but very high quality ones in the future. %Thus. there mayThus, there may be smaller tiles in the set of $A_{\alpha,k}$ for the chunk $k$ in the near future compared to the distant future. Hence, smaller amount of bandwidth may be required for the chunks of near future.

We obtain
\begin{theorem}
The algorithm 360-ROBUST gives a feasible solution of the problem $\mathcal{P}_{\mathrm{eq}}$. The stall time does not increase compared to the optimal solution of the relaxed problem.
\end{theorem}
Note that if the quantization levels are very close, then the feasible solution obtained will be very close to the optimal solution. Also note that Algorithm 360-ROBUST scales linearly with the number of chunks. %If the quantization levels are minute, the algorithm closely matches the optimal solution. Also note that the stall time remains the same as in the relaxed problem.
%\vspace{-.1in}
%We, now, compute the optimality gap of Algorithm 360-ROBUST.
%\begin{theorem}\label{thm:opt_gap1}
%Suppose the optimal value of the objective function (QoE) in $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ is $\mathrm{OPT}$.
%The value of the objective  function attained by Algorithm 360-ROBUST is at least
%\begin{align}
%\mathrm{OPT}-\max_{j\in {0,\ldots,m-1}}K(U(R_{j}+\dfrac{R_{j+1}-R_{j}}{K})-U(R_{j})).
%\end{align}
%\end{theorem}
%
%%\feng{[[Provide some intuitions of the above theorem.]]}
%
%The above theorem provides the bound on the QoE gap attained by the Algorithm 360-ROBUST as compared to the optimal value.  Note from the second part of Proposition~\ref{prop:convexrobust} that the optimal value of the relaxed version $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$ is greater than or equal to the optimal value of the exact  one $\mathcal{P}_{\mathrm{eq}}$. Thus, the difference between the  value of the objective function provided by Algorithm 360-ROBUST and that of the optimal value of the exact problem $\mathcal{P}_{\mathrm{eq}}$ is {\em at most} 
%\begin{align}
%\max_{j\in {0,\ldots,m-1}}K(U(R_{j}+\dfrac{R_{j+1}-R_{j}}{K})-U(R_{j})).
%\end{align}
%
%The proof is deferred to  the supplementary paper owing to the space constraint. The above also shows that the optimal QoE gap is small when the quantization gaps are small, {\em i.e.}, the difference between $R_{j+1}$ and $R_{j}$ are small for all $j\in 0,\ldots, m-1$.  Note that if the utility function is linear, the optimality gap is independent of the number of chunks. Specifically:
%\begin{corollary}
%If $U(\cdot)$ is linear ($U(x)=x$), the value attained by Algorithm 360-ROBUST is at least
%\begin{align}
%\mathrm{OPT}-\max_{j\in {0,\ldots,m-1}}(R_{j+1}-R_{j})
%\end{align}
%\end{corollary}
%\fengout{Hence, Algorithm \textbf{360-ROBUST} yields a solution which is more likely to be bounded by the maximum difference of the two immediate quantization level of the rate. However, if the utility function is non-linear it is a function of the number of chunks.}

%\feng{[[Given the above gap, so what? Do you evaluate how large it is in experiments? Give some forward pointer.]]}

\subsection{Online Algorithm}
Based on the offline algorithm, we now propose the online algorithm which will adapt to the variation of the bandwidth and FoV dynamically, both of which cannot be perfectly predicted, at runtime. In the online version, the algorithm will decide the rate at which tiles will be downloaded for the immediate next chunk. We consider Receding Horizon Control (RHC)  or {\em sliding window} control type algorithm with a forward-looking window size of $W$ chunks.

Specifically, when the tiles of the $c$-th chunk are being fetched, the online algorithm calculates the download rates $\gamma_k$ for chunks $k=c+1, \ldots,c+W$ by solving the following optimization problem:
\begin{eqnarray}
\mathcal{P}^{\mathrm{online}}_{\mathrm{eq}}: & \text {maximize } &\sum_{k=c+1}^{c+W}U(\gamma_k)-\lambda(\tilde{t}_{W+c}-(W+c-1)L-t_{\mathrm{c}})\nonumber\\ & &-\eta\sum_{k=c+1}^{c+W}|\gamma_{k}-\gamma_{k-1}|\nonumber\\
& \text{subject to } &  (\ref{eq:equi}), (\ref{eq:downtime}), (\ref{eq:max_buffer})\nonumber\\
%& & \gamma_k\leq R_{j,k} \forall j\in \mathcal{A}_{\alpha}\label{eq:robust_constraint}\\
& \text{var}: & \gamma_k\in \{R_0,\ldots, R_{m}\}\nonumber
\end{eqnarray}

%\feng{[[Comment on the objective function. How different is it from the offline version besides only looking at next $W$ chunks?]]}

The time horizon is limited we only want to obtain an optimal solution for $W$ chunks ahead. In $\mathcal{P}^{\mathrm{online}}_{\mathrm{eq}}$, $\gamma_{c}$ is the minimum rate among the tiles of the set $A_{\alpha,c}$ to be downloaded. $t_{c}$ is the time at which the $c$-th chunk will stop downloading. The $c+1$-th chunk can only start downloading at time $t_{c+1}$.
%
The algorithm runs after each chunk download to determine the quality for the next chunk.
%~\cite{mpc}
The receding horizon control has advantages compared to the fixed horizon control, as it can adapt to the changes dynamically after each chunk. %Since this is a sliding window protocol, we optimize after each chunk has been downloaded with new prediction of the FoV and the bandwidth. %Note that the width of chunk is small (in the order of few seconds), hence the optimization problem $\mathcal{P}^{\mathrm{online}}_{\mathrm{eq}}$ needs to be solved very frequently.   %Hence, it will take at least $L+W_k$ time to play the $k$-th chunk. The expectation is taken over the new distribution depending on the head movements.

\textbf{The algorithm}: Similar to the offline scenario, we first relax the integer constraint to obtain the convex relaxation version of the problem. Subsequently, we obtain the optimal solution. Finally, we employ Algorithm 360-ROBUST to obtain the feasible solution. We only have to employ the algorithm for $c+W$  chunks starting from chunk $c+1$ instead of running the algorithm from $k=1$ to $K$. In the following, we discuss how we predict the bandwidth and the FoV in an online manner. %how to adapt dynamically   in order to achieve better results in face of the bandwidth prediction error and the FoV prediction error.
%It is easy to discern that the Algorithms ~\ref{algo2}, \ref{algo3}, and \ref{algo4} can be easily adapted to the online version with $W+c$ in place of $K$. Because of the low complexity nature of the Algorithms~\ref{algo2}, \ref{algo3}, and \ref{algo4}, they can be easily adapted for solving the online version repeatedly. Recall that Algorithm~ \ref{algo2} is obtained from solving the relaxed version of the problem by relaxing the discrete strategy space.

\textbf{Bandwidth Prediction}: Note that in the online algorithm, we assume that the bandwidth can be estimated for $W$ chunks ahead. However, if the bandwidth estimation is erroneous, then we have to account for that error. We download all the tiles of the first chunk  at the base layer $R_0$ in order to estimate the bandwidth. This will help to build up the buffer so we can apply our proposed algorithm. The bandwidth for the future after time $t$ is predicted as the harmonic mean of the observed values till  time $t$. A similar approach has been used in previous non-360 video streaming systems \cite{yin,jiang}. 
%Estimating the bandwidth as a harmonic mean seems to work well for video streaming, as has been studied in


% when the buffer has at least $\eta$ chunks to obtain the optimal download rates of the tiles in a chunk.

While downloading the $k$-th chunk, if the bandwidth is higher than the estimated one, we do not increase the rate. Instead, we use ithe additional bandwidth to download later chunks. %On the other hand, if the download is lower than the estimated one, we do not change the Note that once the chunk $k$ is being downloaded,  we do not optimize for $k$-th chunk. However, the bandwidth may be very bad while downloading the chunk $k$ which may result in a  stall. We can minimize it by getting all the tiles only in the base layer\footnote{If we are using the SVC, then we can ignore the enhancement layers and stop downloading all the enhancement layers.}. 

%On the other hand, if the bandwidth is high compared to the estimated value, we do not increase the download rate, rather we keep downloading the $k$th chunk at the same  rate at which it is being fetched.  The additional bandwidth is used to optimize the rates starting from chunk numbered $k+1$. % The window size $W$ has to be chosen judiciously. Note that if the bandwidth has a strong temporal correlation $W$ should be small in order to obtain optimal v. However, if the bandwidths are i.i.d., $W$ should be large.  %We can solve the problem of bandwidth prediction error by making the criteria that the first $\eta$ tiles need to be downloaded at the base layer before using our proposed algorithms as we mentioned in Section IV-B. %Note that in the online algorithm, we assume that the bandwidth can be estimated for $W$ chunks ahead. However, if the bandwidth estimation is erroneous, then we have to account for that error. We will make all the tiles of the first $\eta$ chunks have to be downloaded at the base layer $R_0$. This will help to build the buffer and then we can apply our heuristic algorithm to obtain the optimal download rates of the tiles in a chunk.

%\feng{[[The above paragraph is unclear -- I don't know what you want to say. Consider removing it.]]}

%Note that once we decide the rates at which the chunk $i$ to be downloaded, we do not change it in the online approach. However, the bandwidth may be very bad while downloading the chunk $i$ which may result into the stall. We can minimize it by getting all the tiles only in the base layers\footnote{If we are using the SVC, then we can ignore the enhancement layers and stop downloading all the enhancement layers.} if the buffer does not have at least $\eta$ chunks ahead. On the other hand, if the bandwidth is high compared to the estimated value, we do not increase the download rate, rather we keep downloading the $i$th chunk. We then download the tiles of future chunks at a higher rate.

\textbf{FoV prediction}: In the optimization problem we try to fetch the tiles which have high probability to be part of the FoV. Hence, the user may watch the same quality video. Thus, our algorithm is robust in providing the same play-back rate with a high probability. Thus, the impact of the FoV prediction error will be low. 
%\feng{[[The above argument doesn't make sense. If the FoV prediction is inaccurate, how can you fetch in-FoV tiles with high probability? I think you should cite existing papers showing that FoV prediction can be done at a reasonable accuracy.]]}
%
%\feng{[[The text below is very unclear. Need to rewrite it completely.]]}
However, a user's FoV may not consist of tiles which are not in the part of $\mathcal{A}_{\alpha,c}$ for the current chunk $c$, {\em the user can still watch the video in the base layer. } Hence, there will be no stall or ``black screen". 

For the future chunks, the set $\mathcal{A}_{\alpha,k}$, $k=c+1,\ldots, c+W$ is adapted with based on the current FoV.   The estimation is adjusted after each frame is downloaded. Specifically, we set an weight $1-x_k$ ($0\leq x_k\leq 1)$ on the current FoV for chunk $k$ and  put an weight $x_k$ on the empirical distribution of the FoV calculated before through crowd-sourcing. Specifically, in the online version, the set $\mathcal{A}_{\alpha,k}$ is updated in the following manner: we put probability $1-x_c$ on the set of tiles within the FoV for the chunks $c+1,\ldots, c+W$ and put the probability $x_c$ on the crowd sourced empirical distribution of the FoV for the chunks $c+1,\ldots, c+W$. The set $\mathcal{A}_{\alpha,k}$ is then computed for chunks $k=c+1,\ldots, c+W$.  %In the next section, we empirically evaluate the optimal $W$ and $x_k$ through trace-driven emulation result. 
%each which consists of the tiles if the online algorithm has to decide the download rate starting from chunk $c+1$. We put the probability $x_k$ on the empirical distribution of the FoV.

%The window size $W$ can be varied dynamically. If a user's FoV has a short time correlation, the $W$ is kept at a small value. However, if the FoV changes abruptly, or uncorrelated, the $W$ is kept at a large value.



%It is needless to say that if the quantization gaps are small, Algorithm~\ref{algo2} will provide a solution closer to the optimal one.
%
%\subsection{Optimal Algorithm for a class of utility function}\label{sec:optimal}
%In the previous section, we describe a simple heuristic algorithm which gives a feasible solution from the relaxed problem. The algorithm performs good if there is a continuum of the achievable rates. However, in practice this may not happen.  In the following, we describe an algorithm (Algorithm~\ref{algo3})  for selecting the download rates for tiles in a chunk and we show that the algorithm is optimal even for the original problem $\mathcal{P}_{\mathrm{eq}}$ for a class of utility functions under some assumptions which frequently arise in practice. The algorithm also has only polynomial complexity in the number of chunks, hence, can be computed efficiently.  %The other advantage of Algorithm~\ref{algo3} is that
%\begin{figure}
%		%\vspace{-.15in}
%	
%\begin{algorithm}[H]
%\small
%\begin{algorithmic}
%\STATE {\bf Initialization:} $\gamma_k=R_0$ for all $k$.
%\FOR{$k=1,\ldots, K$}
%%\STATE $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
%\STATE Compute $t_k$ according to (\ref{eq:downtime}).
%\ENDFOR
%\IF{$t_{K}\geq (K-1)L+t_{\mathrm{ini}}$}
%\STATE Exit.
%\ENDIF
%\STATE $\gamma^{\prime}_{k}=\gamma_k$; $t^{\prime}_k=t_k$ for all $k$.
%\FOR{$k=1,\ldots, K$}
%\FOR{$j=1,\ldots, m$}
%\STATE Set $\gamma^{\prime}_{k}=R_j$. %for all $i\in \mathcal{A}_{\alpha,k}$.
%\FOR{$f=k,\ldots, K$}
%\STATE Compute $t^{\prime}_{f}=t^{\prime}_{f-1}+\dfrac{L(|\mathcal{A}_{\alpha,f}|\gamma^{\prime}_f+|\mathcal{A}^{C}_{\alpha,f}|R_0)}{C_f}$.
%\ENDFOR
%\IF{$t_K\leq (K-1)L+t_{\mathrm{ini}}$}
%\STATE Set $\gamma_k=\gamma^{\prime}_k$.
%\STATE Update $t_{k}=t^{\prime}_{k}$.
%\ENDIF
%\ENDFOR
%%\STATE Update $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
%\ENDFOR
%\end{algorithmic}
%\caption{An optimal algorithm for  $\mathcal{P}_{\mathrm{eq}}$ when $\eta=0$, $U(\cdot)$ is linear, and Assumption~\ref{assum:ordering} hold.} \label{algo3}
%\end{algorithm}
%%\vspace{-0.4in}
%\end{figure}
%%\begin{algorithm}
%%$R_{i,k}=R_0$ for all $i$ and $k$\;
%%$R^{\prime}_{i,k}=R_{i,k}$ for all $i$ and $k$\;
%%\For{$k=1,\ldots, K$}{
%%Compute $t_k$ according to (\ref{eq:tk})\;
%%}
%%\If{$t_{K}\geq (K-1)L+t_{\mathrm{ini}}$}{Exit\;}
%%\For{$k=1,\ldots, K$}{
%%\For{$j=1,\ldots, m$}{
%%Set $R^{\prime}_{i,k}=R_j$ for all $i\in \mathcal{A}_{\alpha,k}$\;
%%\For{$a=k,\ldots, K$}{
%%Compute $t_{a}=t_{a-1}+L\dfrac{\sum_{i}R^{\prime}_{i,a}}{C_a}$\;
%%}
%%\If{$t_K\leq (K-1)L+t_{\mathrm{ini}}$}{
%%Set $R_{i,k}=R^{\prime}_{i,k}$ for all $i$\;
%%}
%%}
%%}
%%\caption{Algorithm 3}\label{algo3}
%%\end{algorithm}
%%\textbf{Algorithm 3}:
%%\begin{enumerate}
%%\item Initialization: $R_{i,k}=R_0$ for all $i$ and $k$.
%%\item Set $R^{\prime}_{i,k}=R_{i,k}$ for all $i$ and $k$.
%%\item For $k=1,\ldots, K$
%%\item Compute $t_k$ according to (\ref{eq:tk}).
%%\item End For.
%%\item If $t_{K}\geq (K-1)L+t_{\mathrm{ini}}$, then exit.
%%\item Else: For $k=1,\ldots,, K$ do the following
%%\begin{enumerate}
%%\item For $j=1,\ldots, m$
%%\item Set $R^{\prime}_{i,k}=R_j$ for all $i\in \mathcal{A}_{\alpha,k}$.
%%\item For $l=k,\ldots, K$
%%\item Compute $t_l=t_{l-1}+L\dfrac{\sum_{i}R^{\prime}_{i,l}}{C_l}$.
%%\item End For.
%%\item If $t_K\leq (K-1)L+t_{\mathrm{ini}}$,
%%\item Then: Set $R_{i,k}=R^{\prime}_{i,k}$.
%%\item Else : Exit the inner loop.
%%\item End For.
%%\end{enumerate}
%%\item End For.
%%%\item Compute $\tilde{t}_1, \tilde{t}_2$Rank in the non-increasing order according to $\dfrac{U(R_{i})}{\sum_{j\in \mathcal{A}_{\alpha}}R_i+R_0}$ for each $i$ and $k$.
%%%\item For $k=1,\ldots, K$, we have
%%%\item $R_{j,k}=R_{i}$ for $j\in \mathcal{A}_{\alpha}$.
%%\end{enumerate}
%The run-time complexity of Algorithm~\ref{algo3} is $O(K^2)$. Thus, it is quadratic in the number of chunks. Hence, it is easily implementable.
%
%Recall from (\ref{eq:tk})  that $t_k$ is the start time of downloading chunk $k$. In  Algorithm~\ref{algo3}, first all the tiles are fetched at the base rate $R_0$. Even such a small rate introduces the stall, then, the optimal solution is reached as we put large weight on minimizing the stall time. If there is no stall, then,  for each chunk, the rate $\gamma_k$ is increased gradually (by assigning to $\gamma^{\prime}_k$) until it introduces a stall. The algorithm does the same for each subsequent chunk. The algorithm is very simple to implement. Note that  Algorithm~\ref{algo3} {\em only} fetches the tiles at a higher quality within the set $\mathcal{A}_{\alpha,k}$ for chunk $k$. It {\em does not fetch} all the tiles  within chunk $k$ at a higher rate.
%
%The algorithm is a greedy type where it tries to fetch the current chunk at the highest possible rate rather equalizing the rates among various chunks.
%The cardinality of $\mathcal{A}_{\alpha,k}$ is higher if $\alpha$ is high or the distribution of the FoV estimation has a higher variance. Thus, if there is a higher variance regarding the FoV, the algorithm needs to fetch more tiles in order to guarantee a rate with probability $\alpha$.
%
%%Note that one drawback of the above approach is that the qualities may vary over different chunks. For example, if the future bandwidth is very poor, it will fetch the tiles at a lower qualities; though it can fetch the tiles of the current chunk at a higher rate as the current bandwidth is high. %To avoid the above, one can reduce the maximum rate one can fetch the tiles for current chunks and use the residual bandwidth for downloading tiles not belonging to $\mathcal{A}_{\alpha,k}$.
%
%%In the online version, we only optimize for some $W$ chunks ahead ($W<K$). Thus, the online version can be computed very fast. %To avoid that, one approach can be to restrict the maximum possible rate for the chunks of the near future at some lower rates.
%
%In the following we show that the above algorithm is optimal under some assumptions.
%%\vspace{-.1in}
%\begin{assumption}\label{assum:ordering}
%$|\mathcal{A}_{\alpha,k}|\geq |\mathcal{A}_{\alpha,k-1}|$ for all $K\geq k\geq 2$.
%\end{assumption}
%Recall that the FoV is estimated. The above assumption entails that the estimate is assumed to be more accurate in near future rather than the distant one as we need fewer tiles to cover the FoV with probability $\alpha$. In practice, we also commonly observe that the prediction is more accurate in the near future compared to the distant future \cite{bao}. Hence, the high probability region should consist of fewer tiles in the near future compared to the distant ones. %Hence, it is more likely that few tiles are required to constitute the high visibility region for chunks in the near future.
%
%We, further, assume that the utility varies linearly with rate. More formally,
%%\vspace{-.1in}
%\begin{assumption}\label{ref:linearutility}
%$U(x)=ax+b$, where $a$, $b$ are constant.
%\end{assumption}
%The following theorem states that Algorithm~\ref{algo3} is optimal if Assumptions~\ref{assum:ordering} and \ref{ref:linearutility} hold. Note that the utility function satisfies Assumption 1.
%%Assumption~\ref{ref:linearutility} entails that the utility varies linearly with the rate.
%\begin{theorem}\label{thm:optimal}
%Algorithm~\ref{algo3} provides an optimal solution of $\mathcal{P}_{\mathrm{robust}}$ if Assumptions~\ref{assum:ordering} and \ref{ref:linearutility} hold, $\eta=0$, and $\lambda$ is large enough\footnote{Formally, $\lambda>\sum_{k=1}^{K}U(R_{max})$}.
%\end{theorem}
%\begin{proof}
%Suppose $R_{i,k}$, $\gamma_k$ for $k=1,\ldots, K$  are obtained using Algorithm~\ref{algo3}. We prove the theorem using Induction.
%
%For $K=1$:
%Note that Algorithm~\ref{algo3} always checks whether the stall time increases before fetching higher quality tiles of the chunk. Hence, Algorithm~\ref{algo3} gives the highest possible rate by keeping the stall time minimum. Since $\lambda$ is large enough, thus, it is optimal for $K=1$. % for all $i\in \mathcal{A}_{\alpha,k}$ and $k\in \{1,\ldots, K\}$.
%
%Now suppose that the statement true for $K=k$, we now show that it is true for $K=k+1$. Suppose not, {\it i.e.}, it is not optimal for $K=k+1$.
%
%Specifically, there exists $\gamma^{\prime}_{j}$ for $j=1,\ldots, k+1$ which can give a higher objective value compared to Algorithm~\ref{algo3}. Note that since $\lambda$ is large enough, thus, the stall time should not increase compared to the solution $\gamma_j$.
%
%%Note that $\gamma^{\prime}_j=\min\{R^{\prime}_{i,j}: i\in \mathcal{A}_{\alpha,j}\}$.
%%
%%The total utility obtained from the solution given by Algorithm~\ref{algo3} is
%%\begin{align}
%%\sum_{j=1}^{k+1}R_{i,j}
%%\end{align}
%% The total utility obtained from the solution $R^{\prime}_{i,j}$ is
%% \begin{align}
%%\sum_{j=1}^{k+1} R^{\prime}_{i,j}
%%\end{align}
%%Hence, we must have
%%\begin{align}
%%\sum_{j=1}^{k+1}R^{\prime}_{i,j}>\sum_{j=1}^{k+1}R_{i,j}.
%%\end{align}
%%Since the statement is true for $K=k$, we must have
%%\begin{align}
%%\sum_{j=1}^{k}R^{\prime}_{i,j}\leq\sum_{j=1}^{k}R_{i,j}.
%%\end{align}
%Because of the linear utility, the utility attained by Algorithm~\ref{algo3} is
%\begin{align}
%\sum_{j=1}^{k+1}\gamma_j.
%\end{align}
%Similarly, the utility attained by the solution $\gamma^{\prime}_{j}$ is
%\begin{align}
%\sum_{j=1}^{k+1}\gamma^{\prime}_j
%\end{align}
%Since $\gamma^{\prime}_j$ gives a higher QoE and $\eta=0$, thus,
%\begin{align}\label{eq:gam1}
%\sum_{j=1}^{k+1}\gamma^{\prime}_j>\sum_{j=1}^{k+1}\gamma_j.
%\end{align}
%
%Since we already assumed that the statement is true for $K=k$,  thus, $\gamma_j$ is optimal for $K=k$. Thus, we must have
%\begin{align}\label{eq:gam2}
%\sum_{j=1}^{k}\gamma^{\prime}_j\leq \sum_{j=1}^{k}\gamma_j.
%\end{align}
%%\end{align}However, from
%%\begin{align}\label{eq:gam}
%%\gamma^{\prime}_{k+1}+\sum_{j=1}^{k}\gamma^{\prime}_j>\gamma_{k+1}+\sum_{j=1}^{k}\gamma_j
%%\end{align}
%The total bits to be downloaded for the solution $\gamma^{\prime}_{j}$ is
%\begin{align}\label{eq:bit}
%L[\sum_{j=1}^{k+1}|\mathcal{A}_{\alpha,j}|\gamma^{\prime}_j+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|]
%\end{align}
%Since it does not increase the stall time, thus, the above number of bits can be downloaded within the deadline $t_{k+1}$.
%Now,
%\begin{align}\label{eq:inequal}
%\gamma^{\prime}_{k+1}|\mathcal{A}_{\alpha,k+1}|-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k+1}|\nonumber\\
%\leq \gamma^{\prime}_{k+1}|\mathcal{A}_{\alpha,k+1}|-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k}|
%\end{align}
%where the last inequality follows from (\ref{eq:gam2}) and Assumption~\ref{assum:ordering}. Hence, the total number of bits that can be downloaded if $\gamma_{k+1}=\gamma^{\prime}_{k+1}-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)$ is given by
%\begin{align}
%& L[\gamma^{\prime}_{k+1}|\mathcal{A}_{\alpha,k+1}|-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k+1}|+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|\nonumber\\& +\sum_{j=1}^{k}\gamma_j|\mathcal{A}_{\alpha,j}|]
%\end{align}
%Hence, from (\ref{eq:inequal}) and Assumption~\ref{assum:ordering} the above expression can be upper bounded by
%\begin{align}
%& L[\gamma^{\prime}_{k+1}|\mathcal{A}_{\alpha,k+1}|-\sum_{j=1}^{k}\gamma_j|\mathcal{A}_{\alpha,k}|+\sum_{j=1}^{k}\gamma_j|\mathcal{A}_{\alpha,j}|+\nonumber\\& \sum_{j=1}^{k+1}\gamma^{\prime}_j|\mathcal{A}_{\alpha,j}|+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|]\nonumber\\
%& \leq L[\gamma^{\prime}_{k+1}|\mathcal{A}_{\alpha,k+1}|+\sum_{j=1}^{k}\gamma^{\prime}_j|\mathcal{A}_{\alpha,j}|+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|]
%\end{align}
%where the last inequality again follows from Assumption~\ref{assum:ordering}. However, the above expression is exactly equal to (\ref{eq:bit}), thus, the utility attained in the $k+1$th chunk without increasing the stall time is $\gamma^{\prime}_{k+1}-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)$. Thus, the utility attained by the solution given in Algorithm~\ref{algo3} is at least
%\begin{align}
%\sum_{j=1}^{k+1}(\gamma_{j}-\gamma_j+\gamma^{\prime}_j)+\gamma^{\prime}_{k+1}=\sum_{j=1}^{k+1}\gamma^{\prime}_{j}
%\end{align}
%which contradicts (\ref{eq:gam1}). Hence, the statement is true for $K=k+1$ assuming that it is true for $K=k$.
%
%Thus, from the principle of mathematical induction the result follows.
%
%	\end{proof}
%
%%\begin{proof}
%%See Appendix~\ref{sec:proof}.
%%Thus, using Algorithm~\ref{algo3} the following number of bits can be downloaded within the deadline $t_{k+1}$
%%\begin{align}
%%L[\gamma^{\prime}_{k+1}-\sum_{j=1}^{k}(\gamma_j-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k}||\mathcal{A}_{\alpha,j}|\gamma^{\prime}_
%%\end{align}
%%Hence, from (\ref{eq:gam}) the total number of bits to be downloaded must be
%%\begin{align}
%%>L[\sum_{j=1}^{k}|\mathcal{A}_{\alpha,j}|\gamma^{\prime}_j+\sum_{j=1}^{k}(\gamma_{j}-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k+1}|+\gamma_{k+1}\mathcal{A}_{\alpha,k+1}+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|]
%%\end{align}
%%Since $|\mathcal{A}_{\alpha,j}|\leq |\mathcal{A}_{\alpha,j+1}|$, thus, the total number of bits to be downloaded by Algorithm~\ref{algo3} up to chunk $k$ is
%%\begin{align}
%%\leq L[\sum_{j=1}^{k}|\mathcal{A}_{\alpha,j}|\gamma^{\prime}_j+\sum_{j=1}^{k}(\gamma_{j}-\gamma^{\prime}_j)|\mathcal{A}_{\alpha,k}+\gamma_{k+1}\mathcal{A}_{\alpha,k+1}+\sum_{j=1}^{k+1}R_{0}|\mathcal{A}^{C}_{\alpha,j}|]
%%\end{align}
%%Hence, the total number of bits to be downloaded by Algorithm~\ref{algo3} compared to the solution $R^{\prime}_{i,k}$ is always less. Hence, the highest utility that can be gained from the solution $R^{\prime}_{i,k}$ without increasing the stall time is
%%\begin{align}
%%\sum_{j=1}^{k+1}\gamma_{j}
%%\end{align}
%%which contradicts that the solution $R^{\prime}_{i,k}$ gives a higher utility compared to Algorithm~\ref{algo3}. Hence, the result follows.
%%Since the stall time does not increase, hence, the total number of bits that can be downloaded is
%%\begin{align}
%%>L\gamma_{k+1}\mathcal{
%%\end{align}
%%In Algorithm~\ref{algo3}
%%\begin{align}
%%\sum_{j=1}^{k+1}|\mathcal{A}_{\alpha,j}|\gamma_j+\sum_{j=1}^{k+1}R_0|\mathcal{A}^{C}_{\alpha,j}|.
%%\end{align}
%%Note that $|\mathcal{A}_{\alpha,j+1}|\geq |\mathcal{A}_{\alpha,j}|$. Hence,
%%\begin{align}
%%\sum_{j=1}^{k+1}|\mathcal{A}_{\alpha,j}|\gamma^{\prime}_j>sum_{j=1}^{k+1}|\mathcal{A}_{\alpha,j}|\gamma_j.
%%\end{align}
%%Thus, less number of bits needed to be downloaded by Algorithm~\ref{algo3}. Since $\gamma^{\prime}_{k+1}>\gamma_{k+1}$, thus, the time required to download the $k+1$th chunk is higher compared to Algorithm~\ref{algo3}. However, from (\ref{eq:gam}) note that
%%\begin{align}
%%(\gamma^{\prime}_{k+1}-\gamma_{k+1})|\mathcal{A}_{\alpha,k+1}|>\sum_{j=1}^{k}|\mathcal{A}_{\alpha,k}|(\gamma_{j}-\gamma^{\prime}_j)
%%\end{align}
%%which contradicts that . Hence, the result follows.
%%\end{proof}
%
%%\begin{proof}
%%Before proving the theorem we need one more result.
%%\begin{lemma}
%%For a given sum of the utilities i.e. $\sum_{k=1}^{K}\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$, Algorithm 3 provides the solution which will take the minimum time.
%%\end{lemma}
%%\begin{proof}
%%Suppose not, {\it i.e.}, there exists $R^{\prime}_{i,k}$ which gives the same utility but takes a less amount of time for downloading.
%%
%%Hence,
%%\begin{align}
%%L\sum_{k=1}^{K}\dfrac{\sum_{i=1}^{N}R_{i,k}}{C_k}>L\sum_{k=1}^{K}\dfrac{\sum_{i=1}^{N}R^{\prime}_{i,k}}{C_k}
%%\end{align}
%%Note that the only possibility is that if $\sum_{k=1}^{K}R^{\prime}_{i,k}<\sum_{k=1}^{K}R_{i,k}$. However, this contradicts that the sum of the rates is the same. Otherwise, less number of tiles have to be fetched for attaining the same rate. However, because of the Assumption~\ref{assum:ordering} Algorithm~\ref{algo3} already attains the same rate. Hence, it is not possible.
%%\end{proof}
%%Now, we are ready to prove Theorem~\ref{thm:optimal}.
%%\begin{proof}
%%Suppose $R_{i,k}$ is obtained using Algorithm~\ref{algo3}. We prove the statement using Induction.
%%
%%For $K=1$:
%%Note that algorithm~\ref{algo3} always checks whether the stall time increases before fetching higher quality tiles of the chunk. Hence, it is optimal for $K=1$. % for all $i\in \mathcal{A}_{\alpha,k}$ and $k\in \{1,\ldots, K\}$.
%%
%%Now suppose that it is true for $K=k$, we now show that it is true for $K=k+1$. Suppose not, i.e., it is not optimal for $K=k+1$.
%%
%%Note that the objective value can only be higher if $R^{\prime}_{i,k}$ is higher than $R_{i,k}$ for all $i\in \mathcal{A}_{\alpha,k}$ for some $k\in \{1,\ldots, K\}$. However, since $\lambda$ is large enough, thus, the stall time should not increase compared to the solution $R_{i,k}$.
%%
%%The total utility obtained from the solution given by Algorithm~\ref{algo3} is
%%\begin{align}
%%\sum_{j=1}^{k+1}R_{i,j}
%%\end{align}
%% The total utility obtained from the solution $R^{\prime}_{i,j}$ is
%% \begin{align}
%%\sum_{j=1}^{k+1} R^{\prime}_{i,j}
%%\end{align}
%%Hence, we must have
%%\begin{align}
%%\sum_{j=1}^{k+1}R^{\prime}_{i,j}>\sum_{j=1}^{k+1}R_{i,j}.
%%\end{align}
%%Since the statement is true for $K=k$, we must have
%%\begin{align}
%%\sum_{j=1}^{k}R^{\prime}_{i,j}\leq\sum_{j=1}^{k}R_{i,j}.
%%\end{align}
%%Hence, we must have $R^{\prime}_{i,k+1}>R_{i,k+1}$. However, according to Algorithm~\ref{algo3} there must be some $R^{i,k_1}>R^{\prime}_{i,k_1}$. Now, the additional time total bit to be fetched
%%\begin{align}
%%\sum_{i\in \mathcal{A}_{\alpha,k+1}}(R^{\prime}_{k+1}-R_{k+1})
%%\end{align} Since $|\mathcal{A}_{\alpha,j}|\leq |\mathcal{A}_{\alpha,j+1}|$, hence, for any $j<k+1$ we have
%%\begin{align}
%%\sum_{i\in \mathcal{A}_{\alpha,j}}(R^{\prime}_{k+1}-R_{k+1})\leq \sum_{i\in \mathcal{A}_{\alpha,k+1}}(R^{\prime}_{i,k+1}-R_{i,k+1})
%%\end{align} Now, we must have
%%\begin{align}
%%\sum_{j=1}^{k}\sum_{i\in \mathcal{A}_{\alpha,j}}(R_{j}-R^{\prime}_{k}).
%%\end{align}
%%Note that
%%\begin{align}
%%\sum_{j=1}^{k}\sum_{i\in \mathcal{A}_{\alpha,j}}(R_{j}-R^{\prime}_{j})
%%\end{align}
%%Hence, the result follows. Hence, it must have been that $\mathcal{A}_{\alpha,j}(R_j-R^{\prime}_{j})$
%%\begin{align}
%%R^{\prime}_{i,k+1}-R_{i,k+1}\leq \sum_{j=1}^{k}R_{i,j}-R^{\prime}_{i,j}
%%\end{align}
%%Suppose not. Hence, the time required for downloading is
%%\begin{align}
%%L\sum_{j=1}^{k}\dfrac{R_{i,j}}{C_j}-L\sum_{j=1}^{k}\dfrac{R^{\prime}_{i,j}}{C_j}
%%\end{align}
%%Thus, the complete download time is higher. However, if it does not exceed the stall time, this means that there will be
%%Suppose that $k_1=\arg\min_{j=1,\ldots, k+1}(R^{\prime}_{i,j}>R_{i,j})$. Note that
%%Suppose that it is not true.
%%\textit{Case 2}: $R^{\prime}_{i,k}>R_{i,k}$ for all $i\in \mathcal{A}_{\alpha,k}$ for some $k\in \{1,\ldots,K\}$.
%%
%%The total utility is
%%
%%The total utility attained by Algorithm~\ref{algo3} is
%%Now we must have
%%
%%
%%Suppose that $k_1=\arg\min R^{\prime}_{i,k}>R_{i,k}$. Note that by Algorithm~\ref{algo3}, we must have $R_{i,k}>R^{\prime}_{i,k}$ for some $k<k_1$. However, $|\mathcal{A}_{\alpha,k}|\leq |\mathcal{A}_{\alpha,k_1}|$ as $k<k_1$. Hence, we must have the time taken by  the solution $R^{\prime}_{i,k}$ is greater than or equal to $R_{i,k}$. Hence, the utility can not increase which contradicts that $R^{\prime}_{i,k}$ gives a better objective value. Hence, the result follows. %R_{i,Note from case 1 that if $R^{\prime}_{i,k}>R_{i,k}$ for some $k\in \{1,\ldots, K\}$, then we also must have $R_{i,k_1}>R^{\prime}_{i,k_1}$ for some $k_1\in \{1,\ldots, K\}/\{k\}$. Note that Algrotihm~\ref{algo3} entails that $R^{\prime}_{i,k}<R_{i,k}$ for some $k
%%\end{proof}
%
%The above theorem thus, tells that under reasonable assumptions a simple heuristic algorithm such as Algorithm~\ref{algo3} can be optimal for a large class of utility functions.
%Since $\eta=0$, the QoE provides zero weight on the quality variation across the chunks, hence, the greedy type algorithm such as Algorithm~\ref{algo3} should work better. Intuitively,  Assumption~\ref{assum:ordering} entails that one can gain same utility by consuming lower bandwidth by fetching higher quality tiles  for nearby chunk as it needs to fetch smaller number of tiles compared to the chunks of distant future.  Assumption \ref{ref:linearutility} further characterizes that one will not lose any utility by fetching the best possible quality tiles of the current chunk instead saving the bandwidth for fetching a higher quality tiles for later chunks. %fetching higher quality tiles of the current chunk  compared to  tiles of higher qualities of the distant future. \feng{Why the implications for Assumptions 2 and 4, which just define the rates and the utility functions?}
%
%
%
%%\vspace{-.1in}
%
%\subsection{Heuristic for high $\eta$}
%%\subsection{Near optimal Heuristic for a class of utility functions}
%%The algorithm 3 described in the last section is optimal only for linear utility. In the following we provide another algorithm which also performs good for another class of utility function.
%%
%Algorithm~\ref{algo3} tries to fetch the tiles of the one chunk at the higher rates if there is an excess bandwidth, rather fetching tiles of other chunks at higher rates. Thus, it is only optimal when the weight corresponding to the quality variation among neighboring chunks is zero. One solution is to fetch the tiles of different chunks at similar rates.
%
% %Again, we, first, describe the algorithm.
%\begin{figure}
%		%\vspace{-.15in}
%\begin{algorithm}[H]
%\small
%\begin{algorithmic}
%\STATE {\bf Initialization:} $\gamma_k=R_0$ for all $k$.
%\FOR{$k=1,\ldots, K$}
%%\STATE $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
%\STATE Compute $t_k$ according to (\ref{eq:downtime}).
%%\STATE $t^{\prime}_k=t_k$.
%\ENDFOR
%\IF{$t_{K}\geq (K-1)L+t_{\mathrm{ini}}$}
%\STATE Exit.
%\ENDIF
%\STATE $\gamma^{\prime}_{k}=\gamma_k$ and $t^{\prime}_k=t_k$ for all  $k$.
%
%%\FOR{$k=1,\ldots, K$}
%\FOR{$j=1,\ldots, m$}
%\FOR{$k=K,\ldots,1$}
%\STATE Set $\gamma^{\prime}_{k}=R_j$.
%\FOR{$f=k,\ldots, K$}
%\STATE Compute $t^{\prime}_{f}=t^{\prime}_{f-1}+\dfrac{L(|\mathcal{A}_{\alpha,f}|\gamma^{\prime}_f+|\mathcal{A}^{C}_{\alpha,f}|R_0)}{C_f}$.
%\ENDFOR
%\IF{$t_K\leq (K-1)L+t_{\mathrm{ini}}$}
%\STATE Set $\gamma_k=\gamma^{\prime}_k$.
%\STATE Update $t_{k}=t^{\prime}_{k}$.
%\ENDIF
%\ENDFOR
%%\STATE Update $\gamma_k=\min\{R_{i,k}:i\in \mathcal{A}_{\alpha,k}\}$.
%\ENDFOR
%\end{algorithmic}
%\caption{A heuristic for $\eta$ is large (close to $1$).}\label{algo4}
%\end{algorithm}
%%\vspace{-0.3in}
%\end{figure}
%%\begin{algorithm}\label{algo4}
%%
%%\end{algorithm}
%%\begin{enumerate}
%%\item Initialization $R_{i,k}=R_0$ for all $i$ and $k$.
%%\item Set $R^{\prime}_{i,k}=R_0$ for all $i$ and $k$.
%%\item For $j=1,\ldots,m$
%%\begin{enumerate}
%%\item For $k=1,\ldots, K$
%%\item Set $R^{\prime}_{i,k}=R_j$, $\forall i\in \mathcal{A}_{\alpha,k}$.
%%\item For $l=k,\ldots,K$
%%\item Compute $t_l=t_{l-1}+L\dfrac{\sum_{i}R^{\prime}_{i,l}}{C_l}$.
%%\item End For.
%%\item If $t_{K}\leq (K-1)L+t_{\mathrm{ini}}$,
%%\item Set $R_{i,k}=R^{\prime}_{i,k}$.
%%\item End for.
%%%\item $R_{i,k}=R_{j}$  $\forall j\in \mathcal{A}_{\alpha,if $\tilde{t}_k\leq (k-1)L+t_{\mathrm{ini}}$ and $\tilde{t}_K\leq (K-1)L+t_{\mathrm{ini}}$.
%%%\item end for
%%\end{enumerate}
%%\item end for
%%%\item Compute $\tilde{t}_1, \tilde{t}_2$Rank in the non-increasing order according to $\dfrac{U(R_{i})}{\sum_{j\in \mathcal{A}_{\alpha}}R_i+R_0}$ for each $i$ and $k$.
%%%\item For $k=1,\ldots, K$, we have
%%%\item $R_{j,k}=R_{i}$ for $j\in \mathcal{A}_{\alpha}$.
%%\end{enumerate}
%The run-time complexity of Algorithm~\ref{algo4} is $O(K^2)$. Thus, similar to Algorithm~\ref{algo3}, Algorithm~\ref{algo4} scales in quadratic manner with the number of chunks.
%Algorithm~\ref{algo4} first initializes $\gamma_k$ with $R_0$ the minimum possible rate. If there is no stall, the algorithm then tries to increase $\gamma_k$ to the next higher level for all the chunks starting from the last chunk. If it introduces a stall for certain chunk, $\gamma_k$ is not increased for the chunk. The algorithm terminates when the rate can not be increased without introducing the stall for any of the chunks.
%
%Note that Algorithm~\ref{algo4} gives more preference for fetching tiles in the same quality across the chunks. Algorithm~\ref{algo4} tries to equalize the play-back rates across the chunks in contrast to Algorithm~\ref{algo3}. Since Algorithm~\ref{algo4} tries to increase the rate starting from the last chunk, the user is more likely to see a higher quality video as the time passes by.  Thus, Algorithm~\ref{algo4} tries to use the excess bandwidth to fetch higher quality tiles for the later chunks in contrast to Algorithm~\ref{algo3}.
%
%Since Algorithm~\ref{algo4} tries to maintain parity among the rates across the chunks. Hence, the play-back rate variation across the chunks is expected to be lower compared to Algorithm~\ref{algo3}.
%
%
%%In the online version of the algorithm, we only fetch the tiles for some $W$ chunks ahead. However, since we evaluate the scheduling algorithm after downloading each chunk. So, we can expect that the online version of the algorithm will work similar to the offline version for the same estimated bandwidth. % first assigns $R_{i,k}$ with the base layer rate $R_0$, then it fetches the higher quality tiles (say  at rate $R_{j}$)of the chunk $k$ which constitute the set $\mathcal{A}_{\alpha,k}$. Subsequently, it fetches the higher quality tiles ($R_j$) within the set $\mathcal{A}_{\alpha,k+1}$ within the chunk $k+1$  if it does not result into the re-buffering  and so on. Once the next higher quality tiles are fetched, it again start  with fetching the next higher quality tiles (at rate $R_{j+1}$) starting from chunk $k$ and then it proceeds.
%
%%Note that the key difference between Algorithm~\ref{algo4} and Algorithm~\ref{algo3} is that the algorithm 4 only fetches the tiles with higher qualities  of a chunk only if it can fetch the tiles of similar qualities of future chunks. Hence, the algorithm tends to equalize the qualities over the chunks compared to Algorithm~\ref{algo4}. Thus, it is expected that the Algorithm~\ref{algo4} will reduce the quality variation across the chunks. Hence, Algorithm~\ref{algo4} is better suited when there is a larger weight for reducing the quality variation across the chunks.
%%
%%Now, we show that the algorithm provides is optimal within a constant ratio for a class of utility function.
%%
%%
%%\begin{theorem}
%%Let the optimal value of the optimization problem $\mathcal{P}_{\mathrm{robust}}$ be OPT. The value attained by the solution of Algorithm 4 is $\geq \dfrac{1}{2}$OPT if $\lambda$ is large, Assumption~\ref{assum:ordering} is satisfied and the following assumption holds for all $b\in \{1,\ldots,K\}$ and $j=0,\ldots,\max-1$,
%%\begin{align}\label{eq:chunk}
%%\dfrac{U(R_{i+1})}{\sum_{j\in \mathcal{A}_{\alpha,k}}R_{i+1}+\sum_{j\in \mathcal{A}^{C}_{\alpha,k}}R_{0}}\leq \dfrac{U(R_{i})}{\sum_{j\in \mathcal{A}_{\alpha,b}}R_{i}+\sum_{j\in \mathcal{A}^{C}_{\alpha,k}}R_{0}}
%%\end{align}
%%where $\mathcal{A}^{C}_{\alpha,k}$ is the complement of the set $\mathcal{A}_{\alpha,k}$.
%%\end{theorem}
%%Hence, Algorithm 4 provides a solution which achieves at least half of the optimal value if Assumption~\ref{assum:ordering} and (\ref{eq:chunk}) hold.
%%
%%The condition in (\ref{eq:chunk}) seems to be technical, however, {\em it is satisfied by the concave utilities where the rate of increase is very low.} One example for such kind of utility function is $U(x)=x^{a}$ where $0<a<<1$.
%%
%%Intuitively, if the rate of increase of the utility for higher quality tiles are very low, an optimal algorithm should try to fetch the same quality tiles for all the chunks before fetching higher quality ones. Also note that since Assumption~\ref{assum:ordering} holds, thus, the same utility can be achieved with fetching small number of tiles which can result into the total increase in the utility.
%%\vspace{-.1in}
%\subsection{Online Algorithm}
%Now, we describe how to obtain an online algorithms corresponding to the  offline algorithms~\ref{algo2}, \ref{algo3}, and \ref{algo4}. We consider a {\em sliding window} type algorithm. The bandwidth and head movement is predicted for $W$ chunks ahead and then the optimal algorithm is employed for obtaining the optimal download rate for each tile within a chunk.  When the tiles of the $c$-th chunk are being fetched, the online algorithm gives the download rates for chunks $c+1, \ldots,c+W$ by solving the following optimization problem:
%\begin{eqnarray}
%\mathcal{P}^{\mathrm{online}}_{\mathrm{eq}}: & \text {maximize } &\sum_{k=c+1}^{c+W}U(\gamma_k)\nonumber\\ & &-\lambda(\tilde{t}_{W+c}-(W+c-1)L-t_{\mathrm{ini}})\nonumber\\
%& \text{subject to } &  (\ref{eq:equi}), (\ref{eq:downtime}), (\ref{eq:max_buffer})\nonumber\\
%%& & \gamma_k\leq R_{j,k} \forall j\in \mathcal{A}_{\alpha}\label{eq:robust_constraint}\\
%& \text{var}: & \gamma_k\in \{R_0,\ldots, R_{m}\}\nonumber
%\end{eqnarray}
%The $c+1$-th chunk can only start downloading at time $t_{c+1}$. { The algorithm is run after each chunk download to determine the qualities for the next chunk. In practice, it can be run slightly before so that the computational time can be accounted. Such online methods are common in streaming literature \cite{mpc}.}%Since this is a sliding window protocol, we optimize after each chunk has been downloaded with new prediction of the FoV and the bandwidth. %Note that the width of chunk is small (in the order of few seconds), hence the optimization problem $\mathcal{P}^{\mathrm{online}}_{\mathrm{eq}}$ needs to be solved very frequently.   %Hence, it will take at least $L+W_k$ time to play the $k$-th chunk. The expectation is taken over the new distribution depending on the head movements.
%
%It is easy to discern that the Algorithms ~\ref{algo2}, \ref{algo3}, and \ref{algo4} can be easily adapted to the online version with $W+c$ in place of $K$. Because of the low complexity nature of the Algorithms~\ref{algo2}, \ref{algo3}, and \ref{algo4}, they can be easily adapted for solving the online version repeatedly. Recall that Algorithm~ \ref{algo2} is obtained from solving the relaxed version of the problem by relaxing the discrete strategy space.
%
%\textbf{Bandwidth Prediction Error}: Note that in the online algorithm, we assume that the bandwidth can be estimated for $W$ chunks ahead. However, if the bandwidth estimation is erroneous, then we have to account for that error. We download all the tiles of the first $\beta$ chunks at the base layer $R_0$. This will help to build the buffer and then we can apply our proposed algorithm.% when the buffer has at least $\eta$ chunks to obtain the optimal download rates of the tiles in a chunk.
%
%Note that once the chunk $k$ is being downloaded,  we do not change its rate  in the online approach. However, the bandwidth may be very bad while downloading the chunk $k$ which may result in a  stall. We can minimize it by getting all the tiles only in the base layer\footnote{If we are using the SVC, then we can ignore the enhancement layers and stop downloading all the enhancement layers.}. On the other hand, if the bandwidth is high compared to the estimated value, we do not increase the download rate, rather we keep downloading the $k$th chunk at the same pre-fixed rate. Running algorithm to determine fetching for the chunks after $k$ can lead to an increase in the download rate of the future chunks.%We can solve the problem of bandwidth prediction error by making the criteria that the first $\eta$ tiles need to be downloaded at the base layer before using our proposed algorithms as we mentioned in Section IV-B. %Note that in the online algorithm, we assume that the bandwidth can be estimated for $W$ chunks ahead. However, if the bandwidth estimation is erroneous, then we have to account for that error. We will make all the tiles of the first $\eta$ chunks have to be downloaded at the base layer $R_0$. This will help to build the buffer and then we can apply our heuristic algorithm to obtain the optimal download rates of the tiles in a chunk.
%
%%Note that once we decide the rates at which the chunk $i$ to be downloaded, we do not change it in the online approach. However, the bandwidth may be very bad while downloading the chunk $i$ which may result into the stall. We can minimize it by getting all the tiles only in the base layers\footnote{If we are using the SVC, then we can ignore the enhancement layers and stop downloading all the enhancement layers.} if the buffer does not have at least $\eta$ chunks ahead. On the other hand, if the bandwidth is high compared to the estimated value, we do not increase the download rate, rather we keep downloading the $i$th chunk. We then download the tiles of future chunks at a higher rate.
%
%\textbf{FoV prediction error}: Since in the optimization problem we try to fetch the tiles which have high probability to be a part of the FoV. Hence, the user may watch the same quality video with a very high probability.   Thus, the impact of the FoV prediction error will be low. Additionally, note that if the FoV consists of tiles which are not in the part of $\mathcal{A}_{\alpha,k}$, the user can still watch the video in the base layer.
%
%\begin{remark}
%
% We assume the Constant Bit-Rate (CBR) technique where the spatial encoding complexity is constant through the video.  If the encoding complexity is different for different frames we can still achieve a feasible solution using Algorithm 1. However, for Algorithms 2 and 3, we rely on the fact that the bit-rate has to be the same for each chunk. Thus, the characterization of an optimal algorithm even for linear utility for the variable bit rate is a work for the future.
%
%\end{remark}



==> formulation_mobicom.tex <==
\section{Problem Formulation and Equivalent Representation}\label{sec:robust}%
We, first, provide the QoE metric of a user. The QoE is a random variable since the FoV, and the bandwidths are random. Subsequently,  we represent a QoE metric which accounts for the uncertainty. We, finally, formulate the robust optimization problem to maximize the QoE. 
\subsection{QoE Representation}
Let $\mathcal{F}_k$ be the set of tiles within the FoV at chunk $k$. Recall from Section~\ref{sec:system} that $R_{i,k}$ is the rate at which the tile $i$ in chunk $k$ is downloaded. Also recall that to avoid spatial quality variation, all tiles in the FoV of chunk $k$ should  be played at quality $\min_{i\in \mathcal {F}_k}R_{i,k}$. 
%\feng{[[Why due to SVC? AVC is different from this?]]}
Hence, the  utility is governed by the minimum rate among those tiles within the set $\mathcal{F}_k$.
Thus, the video player  wants to maximize $\sum_{k=1}^{K}U(\min_{i\in \mathcal{F}_k}R_{i,k})$.

The video provider wants to reduce the quality variation across the chunks with a high probability. Hence, it wants to minimize the quality variation among the tiles within the FoV across two consecutive chunks. In other words the video service provider wants to minimize
\begin{align}\label{eq:diff1}
\sum_{k=1}^{K-1}|\min_{i\in \mathcal{F}_{k}}R_{i,k}-\min_{i\in \mathcal{F}_{k+1}}R_{i,k+1}|
\end{align}
QoE also decreases as the stall time increases, hence, the QoE metric is given by
\begin{align}\label{eq:qoe}
\text{QoE}= & \sum_{k=1}^{K}U(\min_{i\in \mathcal{F}_{k}}R_{i,k})-\lambda(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})\nonumber\\ & -\eta\sum_{k=1}^{K-1}|\min_{i\in \mathcal{F}_{k}}R_{i,k}-\min_{i\in \mathcal{F}_{k+1}}R_{i,k+1}|
\end{align}
$\lambda$ is the weight factor corresponding to the stall time (cf.(\ref{stall})) and $\eta$ is the weight corresponding to the quality variation across the chunks. 
\begin{remark}
The optimal weights ($\lambda, \eta$) corresponding to different factors of the QoE metric are set depending on the video player's objective. In general those values are often obtained from the user's sensitivity analysis of the stall time duration and the rate-variation across the chunks. %through a learning process. \feng{[[what is the learning process? Learning what?]]}
\end{remark}

\subsection{Robust QoE metric and Problem Formulation}
In the previous subsection, we represent the QoE when the FoV of every chunk is known apriori. However, the FoV evolves randomly with the time depending on the head movement of the user. 
We consider that the video service provider wants to provide a rate $r$ to the users such that the play back rate will be greater than or equal to that rate $r$ with a high probability. % \feng{[[``guaranteed'' contradicts with ``high probability''. Change the presentation.]].}
%
In any kind of entertainment or video streaming, the tail probability is important. If the video quality is poor in even for a small portion of the chunk, it will render poor rating, even though the mean quality is good. Further, the video application would like to serve the FoV using same quality tiles so as not to have quality variations in a chunk affecting QoE. Hence, we need to achieve a trade-off such that the viewing quality is good at least with a certain probability $\alpha$.
%
We, thus, consider a QoE metric where the utility of the user only depends on the rate at least with which the chunk can be viewable with probability $\alpha$.  %\feng{[[Please first define QoE in 360-degree video streaming.]]}
%
Note that such metric is already proposed in the communication channel, or the electricity market.  We, now, formulate a QoE metric, and subsequently, propose solution to maximize the above metric.



%The video service provider wants to maintain stability among the rates across various chunks. The stall time should also be low.
%\vspace{-.1in}
%\subsection{Robust Problem Formulation}
We introduce a notation which we use throughout this section.
\begin{definition}\label{defn:set}
Let $\mathcal{A}_{\alpha,k}$ be the set of tiles of chunk $k$ which has the property that the FoV is a subset of $\mathcal{A}_{\alpha,k}$ with probability at least $\alpha$ for chunk $k$. If there are multiple sets which satisfy the above condition, then, $\mathcal{A}_{\alpha,k}$ is considered to be the set with the lowest cardinality.
Let $\mathcal{A}^{C}_{\alpha,k}$ be the complement of the set $\mathcal{A}_{\alpha,k}$.
\end{definition}
We do not assume that the exact FoV is known beforehand. However, we do assume that the statistics are known. The statistics can be obtained from the crowd sourced data, i.e., FoV distributions different users watching the same video.
%
Also note that in our algorithm we do not need to know the exact distribution, mean, or variance of the FoV. We need to build the set $\mathcal{A}_{\alpha,k}$, the set of tiles which can be viewed with probability $\alpha$.\footnote{Our analysis will go through even if $\alpha$ is different across the chunks.}
%
%\feng{[[$\mathcal{A}_k$ not defined. You only define $\mathcal{A}_{\alpha,k}$.]]}
%
%We do not need the perfect prediction either. In fact, the lack of perfect prediction of the head movement is one of our motivations behind the work. %\feng{[[Mention this in intro -- why we need such a stochastic optimization approach.]]} 

Our QoE metric  is specified for robust optimization technique. We only need to compute the tiles which constitute the set $\mathcal{A}_{\alpha,k}$, the tiles which constitute the set of tiles can be seen with a high probability. %\feng{[[$\mathcal{A}_k$ not defined.]]}


$\mathcal{A}_{\alpha,k}$ is the set of the tiles  which specifies that the FoV will be a subset of this set with probability $\alpha$. Thus, the lowest rate among the tiles of $\mathcal{A}_{\alpha,k}$ gives the lowest rate the user will observe the video with the probability at least $\alpha$. 
%\feng{[[Again, i don't like putting ``guarantee'' and ``probability'' together.]]}

%\feng{[[Why due to SVC? AVC is different from this?]]}
The  utility is considered to be governed by the minimum rate among those tiles within the set $\mathcal{A}_{\alpha,k}$.
Thus, the video player  wants to maximize $\sum_{k=1}^{K}U(\min_{i\in \mathcal{A}_{\alpha,k}}R_{i,k})$. %The above will ensure that the viewers will only see lower qualities with probability $1-\alpha$.

\begin{remark}
	$\alpha$ is a parameter which needs to be determined from the market research.  For robust optimization problems, $\alpha$ is generally taken to be in the interval $[0.9, 0.99]$ \cite{alpha}.
\end{remark}


As stated in Section 4.1, the QoE metric decreases as the rate varies across the chunks (cf. (\ref{eq:diff1})). Hence, the video player wants to minimize the quality variation among the tiles within the set $\mathcal{A}_{\alpha,k}$ across two consecutive chunks. In other words the video service provider wants to minimize 
\begin{align}\label{eq:diff}
\sum_{k=1}^{K-1}|\min_{i\in \mathcal{A}_{\alpha,k}}R_{i,k}-\min_{i\in \mathcal{A}_{\alpha,k+1}}R_{i,k+1}|
\end{align}
Recall from (\ref{eq:qoe}) that QoE also decreases as the stall time increases. Also note from Section 3 that  we assume each tile of every chunk $k$ has to be downloaded at the minimum rate even those tiles are not in the set $\mathcal{A}_{\alpha,k}$ in order to avoid the situation where the user will see block spots when the FoV does not coincide with the exact prediction. Thus, the {\em robust} QoE metric is given by
\begin{align}\label{eq:probust}
\text{QoE}= & \sum_{k=1}^{K}U(\min_{i\in \mathcal{A}_{\alpha,k}}R_{i,k})-\lambda(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})\nonumber\\ & -\eta\sum_{k=1}^{K-1}|\min_{i\in \mathcal{A}_{\alpha,k}}R_{i,k}-\min_{i\in \mathcal{A}_{\alpha,k+1}}R_{i,k+1}|
\end{align}

%\feng{[[I strongly suggest describing the QoE metrics in general (not in the stochastic context) at the beginning of this section (or even using a separate subsection). Then try to formulate the QoE in the stochastic context.]]}


%Hence, the optimization problem that the video service provider wants %utility is the minimum among the rates of the tiles within the set $\mathcal{A}_{\alpha,k}$. %The minimum rate of the tiles within $\mathcal{A}_{\alpha}$ specifies that the video will be seen at least with that rate. The video service provider's objective is now governed with the minimum rate of among the tiles within the set $\mathcal{A}_{\alpha,k}$. If the minimum rate is poor, then, there is a possibility that the quality of service is poor. On the other hand, if the rate is high, the quality of service is also high at least with probability $\alpha.$
Thus, formally, the optimization problem that the video player  is solving is given by
\begin{eqnarray}
\mathcal{P}:\text {maximize } &\sum_{k=1}^{K}U(\gamma_k)-\lambda(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})-\nonumber\\
&\eta\sum_{k=1}^{K-1}|\gamma_{k}-\gamma_{k+1}|\label{eq:robust}\\
\text{subject to } &  (\ref{b_k}), (\ref{eq:tk}), (\ref{eq:max_buffer})\nonumber\\
& \gamma_k= \min_{i\in \mathcal{A}_{\alpha,k}}R_{i,k} \label{eq:constraint}\\
%& d_k=|\min_{i\in \mathcal{A}_{\alpha,k}R_{i,k}-\min_{i\in \mathcal{A}_{\alpha,k+1}R_{i,k+1}|\label{eq:diff}\\
 \text{var}: & R_{i,k}\in \{R_0,\ldots, R_{m}\}\nonumber
\end{eqnarray}
Note from (\ref{eq:constraint}) that $\gamma_k$ denotes the minimum rate of the tiles within the set $\mathcal{A}_{\alpha,k}$.

\begin{remark}
For ease of exposition,  we assume the Constant Bit-Rate (CBR) technique where the spatial encoding complexity is constant through the video.  Our analysis will go through even if the encoding complexity is different for different frames. 
\end{remark}
%\vspace{-.1in}
\subsection{Equivalent Representation}
The constraint set in the optimization problem $\mathcal{P}$ is not in the convex form because of the constraints in (\ref{eq:constraint}) and the discrete strategy space. In the following, we provide equivalent representations of the constraints (\ref{eq:constraint}) which are in convex form. 

Note that in an optimal solution of $\mathcal{P}$ only the tiles within the set $\mathcal{A}_{\alpha,k}$ should be fetched at rates higher than $R_0$ if possible. The rate at which the tiles in the set $\mathcal{A}^{C}_{\alpha,k}$ (recall Definition~\ref{defn:set}) are fetched do not contribute to the utility.  Hence, the tiles in the set $\mathcal{A}^{C}_{\alpha,k}$ is fetched at  rate $R_0$ in an optimal solution. 
 If the tiles within $\mathcal{A}_{\alpha,k}$ are not fetched in the same quality, then, the utility is only governed by the minimum among the rates at which the tiles are fetched. Hence, in an optimal solution  all the tiles in $\mathcal{A}_{\alpha,k}$ at the same rate.  Now, we propose an equivalent representation of the optimization problem.

\begin{theorem}\label{thm:equi}
Suppose that $R^{*}_{i,k}$ is the optimal solution of $\mathcal{P}$. Now, consider the following solution: $R^{\prime}_{i,k}=\min_{i\in \mathcal{A}_{\alpha,k}}R^{*}_{i,k}$ $\forall i\in \mathcal{A}_{\alpha,k}$ and $R^{\prime}_{i,k}=R_0$ $\forall i\in \mathcal{A}^{C}_{\alpha,k}$. Then, $R^{\prime}_{i,k}$ is also an optimal solution.
\end{theorem}
The above theorem will assist us to represent $\mathcal{P}$ in an equivalent form with $\gamma_k$ as decision variables.  Note that the tiles within the set $\mathcal{A}_{\alpha,k}$ $k=1,\ldots,K$  are fetched at rate $\gamma_k$ and the other tiles at rate $R_0$.  We, now, modify the constraints in terms of $\gamma_k$ in place of $R_{i,k}$ for each chunk $k$. First, note that the download time in (\ref{eq:tk}) is modified as
\begin{align}\label{eq:downtime}
t_k=t_{k-1}+\dfrac{L(|\mathcal{A}_{\alpha,k}|\gamma_k+|\mathcal{A}^{C}_{\alpha,k}|R_0)}{C_k}+\zeta_k,\quad t_0=0.
\end{align}
where $|\cdot|$ denotes the cardinality of the set. 


Finally, we represent the constraint in (\ref{b_k}) as the following:
\begin{align}\label{eq:equi}
& \tilde{t}_k\geq \tilde{t}_{k-1}+L,  \tilde{t}_1\geq t_{\mathrm{ini}} \quad\tilde{t}_k\geq \dfrac{L(|\mathcal{A}_{\alpha,k}|\gamma_k+|\mathcal{A}^{C}_{\alpha,k}|R_0)}{C_k}.
\end{align}
Now, we are ready to represent $\mathcal{P}$ in an equivalent form.
\begin{proposition}
Consider the following optimization problem
\begin{eqnarray}
& \mathcal{P}_{\mathrm{eq}}: \text {maximize } & (\ref{eq:robust})\nonumber\\
& \text{subject to } &  (\ref{eq:equi}), (\ref{eq:downtime}), (\ref{eq:max_buffer})\nonumber\\
%& & \gamma_k\leq R_{i,k} \forall i\in \mathcal{A}_{\alpha,k}\label{eq:robust_constraint}\\
%& & d_k\geq \gamma_k-\gamma_{k+1}\quad d_k\geq \gamma_{k+1}-\gamma_k\nonumber\\
& \text{var}: & \gamma_k\in \{R_0,\ldots, R_m\}\nonumber
\end{eqnarray}
The optimization problem $\mathcal{P}_{\mathrm{eq}}$ is equivalent to (\ref{eq:robust}), and is a discrete optimization problem.
\end{proposition}
%The above result shows that even though the constraint in (\ref{eq:robust_constraint}) is not equal to (\ref{eq:constraint}), yet in any optimal solution $\gamma_k$ must satisfy (\ref{eq:constraint}).

%{\em Outline of the Proof}: $U(\cdot)$ is strictly increasing function. Hence, at the optimal value we must have $\gamma_k$ satisfy constraint (\ref{eq:constraint}). \qed
%\vspace{-.1in}
%\begin{remark}
%The optimization problem $\mathcal{P}_{\mathrm{eq}}$ only gives $\gamma_k$. However, we need the rates $R_{i,k}$. We obtain that in the following manner: if $\gamma_k$ is the optimal solution of $\mathcal{P}_{\mathrm{eq}}$, then we can obtain the optimal rates as follows: $R_{i,k}=\gamma_k$ for all $i\in \mathcal{A}_{\alpha,k}$ and $R_{i,k}=R_0$ for all $i\in \mathcal{A}^{C}_{\alpha,k}$.
%\end{remark}


%\vspace{-.15in}
%\begin{remark}
%%The optimization problem $\mathcal{P}_{\mathrm{eq}}$ is not convex because the decision space is discrete. In the following we propose a relaxed version of the problem which is convex.
% Since $\mathcal{A}_{\alpha,k}$ may be different for different $k$ and there is uncertainty regarding the bandwidth, it is not {\em a priori} clear whether the video service provider should be conservative in the beginning while downloading chunks; which is proved to be a good heuristic to maximize the QoE in the traditional video streaming scenario. \feng{[[I don't think this is always a good heuristic for traditional streaming. Which paper proved that?]]} This is because if $\mathcal{A}_{\alpha,k}$ can be low (thus, fewer amount of bandwidth is required to get a better QoE) for earlier chunks. \feng{[[The last sentence doesn't parse. Overall this remark is unclear. Can we just remove it?]]}
%\end{remark}

%\vspace{-.15in}

%\vspace{-.15in}
%\begin{remark}
%In practice, the user provides a larger weight on the expected play-back rate compared to the play-back rate variation across the chunks, hence, $\eta<1$.
%\end{remark}
%
%\vspace{-.15in}

%\begin{remark}
%Note that the tiles which do not belong to $\mathcal{A}_{\alpha,k}$ are only fetched at the base layer $R_0$. However $R_0$ is strictly  greater than $0$, hence the user still can see those albeit at a lower quality. %at a higher quality compared to $R_{0}$ unless it fetches all the tiles within $\mathcal{A}_{\alpha,k}$. This is because the utility will not increase if the tiles which is not in $\mathcal{A}_{\alpha,k}$.
%\end{remark}

%\vspace{-.15in}
%Thus, $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{robust}}$ can be efficiently solved using existing numerical approaches.


==> intro_mobicom.tex <==
\section{Introduction}
%\vspace{-.1in}
%\subsection{Motivation}
360-degree videos provide users a panoramic view and create a unique viewing experience. These videos are recorded using the omnidirectional cameras. While watching the video, the user can change the viewing direction by moving her head. Typically, the user wearing a VR headset (e.g., the Google Cardboard \cite{cardboard}) can adjust her orientation by changing the pitch, yaw, and roll of the device which corresponds to the X, Y and Z axes, respectively. The field-of-view (FoV) defines the extent of the user's observable portion. It is typically fixed for a VR headset (e.g., 90-degree vertically and 110-degree horizontally \cite{feng}).

The mainstream technologies for streaming 360 videos fetch all panoramic scenes including both the visible and invisible portions\cite{fb,youtube}.
%
Though this is simple, it has some disadvantages. In particular, the bandwidth utilization is high as the chunks of 360-degree videos are of much larger sizes compared to the traditional ones. Thus, if the  bandwidth is low, it will lead to poor viewing quality or stall (rebuffering). Even the wireline capacity may not be enough for HD 360-degree videos \cite{wireline}. Although significant progress has been made in developing VR technologies, the research community still lacks robust bandwidth-efficient streaming algorithms for 360-degree videos for maximizing the QoE of the users.
%
%\fengout{There may be quality variation across different chunks, as different chunks may be fetched at different rates which degrades the quality of experience (QoE).  Hence, without smart algorithms, streaming can easily consume the wireless bandwidth \cite{bandwidthhungry} which leads to degraded QoE. Further, the field-of-view (FoV), and the bandwidth evolve randomly over time. Thus,  without  a robust algorithm, there is no absolute guarantee of the QoE experienced by the user. In the video streaming experience, the tail-index of the video quality distribution often defines the user's QoE.}
%



\if 0

\begin{figure}[hbtp]
\vspace{-0.1in}
\begin{center}
	\includegraphics[width=2in]{360.pdf}
\end{center}
\vspace{-0.1in}
\caption{Adjust viewing direction during 360 degree video playback}
\label{fig:360}
\vspace{-0.1in}
\end{figure}

\fi

%\vspace{-.1in}

% \subsection{Our Contributions}
%In this paper, we propose a robust scheme for tile-based 360 video streaming.
%\fengout{We assume that the 360-degree video service provider wants to maximize the quality of experience (QoE) given the limited bandwidth. The user gets a utility depending on the rate at which a chunk is being downloaded.}
 %We consider that each chunk consists of several tiles.
In a tile-based video streaming,
instead of downloading the entire panoramic view at a same rate, a video player can download the portions of the chunk which are more likely to be viewed at a higher rate.
%
This requires spatially segmenting a 360-degree video chunk into multiple segments called \emph{tiles}. A tile (as opposed to a chunk) is the smallest downloadable content unit.
Tile-based 360 video streaming has been proposed by prior studies~\cite{bao,feng}.  Designing a tile-based streaming algorithm for ABR (adaptive bitrate) 360 videos is very challenging because the algorithm needs to make judicious decisions in both the quality dimension and the spatial (tile) dimension. We note that most existing studies suffer from several limitations.
(1) Bandwidth, and the head movement (thus, FoV) vary randomly over time. However, there lacks a robust algorithm which provides a guarantee on the streaming rate with a high probability regardless of the variation of the head movement, and the bandwidth. % There lacks a robust algorithm which can provide a rate such that the streaming rate degrades below that value with very low probability. 
(2) They mostly take heuristics-based approaches that may lead to suboptimal viewing experiences.
(3) They typically predict \emph{individual} users' head movements to determine which tiles to fetch. Meanwhile, another opportunity for prefetching tiles is to leverage \emph{crowd-sourcing}, i.e., if many other users are interested in viewing a certain direction at certain time, then the corresponding tiles can be prefetched. Despite the simple idea, it is unclear how to incorporate crowd-sourcing into ABR streaming algorithms in a principled manner.
(4) There lacks theoretical rigorousness in terms of maximizing the QoE in the face of fluctuating bandwidth and users' fast head movement.

%\fengout{We assume that the distribution of the FoV can be obtained from the viewing history, the nature of the video, and even from the head movement of the user. Given the distribution of the FoV and the bandwidth estimation, our goal is to design a robust streaming algorithm that maximizes the QoE.}



% However, none of these studies proposed a full-fledged streaming algorithm that adapts the streaming behavior at both the temporal domain (which quality to fetch for each chunk) and the spatial domain (which tiles to fetch for each chunk). Specifically, to the best of our knowledge, our work is the first one to propose a robust video streaming algorithm by considering the variability of both the FoV and the bandwidth.
  % We consider that each tile of a chunk can be encoded at different rates. Each chunk has to be downloaded before its deadline or play time, otherwise a stall will result. Since a user does not want any black spot in the viewing area, we assume that each tile must have to be downloaded at least at the minimum possible rate.  We also assume that the bandwidth can be estimated. Note that the bandwidth determines the download rates of the tiles as higher download rates may increase the stall time if there is not much available bandwidth.

To address the above challenges, our streaming approach introduces a holistic analytical framework built upon the formal method of stochastic optimization. We assume that the user QoE gets a utility based on minimum rate of consumed tiles in each FoV, because the user would like to view all the tiles in the FoV in ideally the same quality to avoid any quality fluctuation. Also the QoE gets penalized when a stall occurs or the inter-chunk quality changes.
%
%\fengout{In order to find a robust optimal algorithm for the QoE we first define the QoE metric which captures the essence of the robustness of the quality. The user's viewing experience depends on the tiles' qualities within the FoV.
%In general, the FoV is governed by the minimum quality of the tiles within the FoV. This is because the user would like to see all the tiles in FoV in the same quality to avoid any quality fluctuation while viewing a chunk. }
%\fengout{where the QoE is considered to be the bit-rate (say, $R$) such that the FoV will be at least that $R$ with probability $\alpha$. The above metric provides the minimum rate $R$ that a user will experience with probability $\alpha$. The parallel can be drawn with the outage capacity in the wireless communication \cite{tse}\cite{out}, where the outage capacity is defined as the rate which can be successfully decoded with probability $\alpha$. In any kind of entertainment or video streaming, the tail probability matters the most. If the video quality is poor in even for a few portion of the chunk, it will render poor  rating, even though the mean quality is good. Hence, we need to achieve a trade-off such that the viewing quality is good at least with a certain probability $\alpha$. Also note that users do not like too much rate variation across the chunks. Hence, the rate variation across the chunks have to be minimized. The  stall duration ({\it i.e.}, the total time the playback's play-out buffer does not have any content to render) should be minimum \cite{yin}.}
%We maximize the play-back rate $R$, and simultaneously minimize the play-back rate variation across the chunks, and the total stall time.
%
We then formulate a stochastic optimization problem by assuming the knowledge of the viewing probability of the tiles. Such probabilities can be easily derived from the combination of crowd-sourced measurements and the FoV prediction of current user performed by 360 video content providers. The formulation jointly
maximizes the consumed bitrate, minimizes the play-back rate variation across chunks, and minimizes the total stall time, based on detailed modeling of the above metrics in the 360 video contexts.
%Note that a smart algorithm should try to fetch current chunks at a relatively lower qualities in order to avoid stalls for the future chunks. Since the FoV prediction is more likely to be accurate for the current chunk rather the future ones. Thus, an algorithm should try to fetch earlier chunks at a higher rate. Hence, finding an algorithm which optimizes the QoE is not {\em a priori} clear and inherently depends on the FoV and the bandwidth prediction}\footnote{\fengout{
 %Since the VR applications are getting popular, users are most likely to watch it on wireless devices such as phones, and tablets. They are mostly mobile. The mobility can affect the stability of the connection. Hence, the bandwidth can vary significantly over the time. Even if the the user is static, the bandwidth can vary depending on how many users are using the channel and the channel gain at a specific time. The number of users, and the channel gain evolve randomly over time. Thus, it is expected that there will be randomness in the bandwidth. Hence, we need an efficient algorithm which considers both the uncertainty in the bandwidth as well the uncertainty in the FoV.}}
%\fengout{In addition, the optimization problem turns out to be non-convex because of the discrete variable space as the available download rates can only take discrete values.}

 %We maximize the above and meanwhile minimize the stall duration. %Hence, we consider the weighted sum of the sum of the playback bit rates of tiles within the FoV and the minimum rate among the tiles in the FoV as our {\em first} QoE  metric.

%
%Optimization over the tail probability has been a concern over the internet. It has been shown that in modern web applications such as Bing, Facebook,
%and Amazon's retail platform, the long tail of latency is of
%particular concern, with 99.9th percentile response times that
%are orders of magnitude worse than the mean. For Amazon,
%a 100ms latency penalty implies a 1\% sales loss \cite{amazon};
%for Google, an additional delay of 400ms in search responses
%reduces search volume by 0.74; and for Bing, 500ms of
%latency decreases revenue per user by 1.2\% \cite{bing}. Thus, such metric measures user engagements and thus improved revenues.
%

%Our objective is to maximize the above QoE metric and the negative of the stall time.  The weight for the stall time is kept very high to ensure that the stall time is always


The above optimization problem turns out to be non-convex because of the discrete variable space, and is therefore difficult to solve.
To address this technical challenge, we first relax the constraints and formulate a relaxed problem that is convex.
%
We then design an algorithm that computes the final scheduling decisions
by strategically mapping the solutions of the relaxed problem back to the original problem. Based on the above algorithms, we then design its online version that can adapt to the fluctuating bandwidth and uncertain head movement at runtime with low overhead incurred.
%\fengout{where the selected bitrate belongs to a set of pre-defined discrete values from the optimal solution of the relaxed convex optimization.
%
%Specifically, the algorithm first down-quantizes the bit-rate of the tiles in order to obtain a feasible downloadable bit-rate. The bandwidth saved by down-quantization is reserved for downloading tiles in next higher bit-rate starting from the last frame if possible. In Theorem~\ref{thm:opt_gap1} we show that such an algorithm provides a constant optimality gap which is independent of the number of chunks.  We also propose an online version of the above algorithms which can adapt the bandwidth or FoV variation dynamically.%if there is an enough bandwidth to fetch all the tiles which constitutes the set of tiles which can be viewed with a probability at least $\alpha$, the algorithm then fetches
%}

%Algorithm~\ref{algo2} may be sub-optimal and a convex optimization problem is required to be solved. We, additionally, provide two algorithms of lower complexities. One (Algorithm~\ref{algo3}) is a greedy type approach where it tries to fetch the tiles of the current chunk at a higher quality rather the subsequent chunks  if there is an excess bandwidth. Intuitively, if the FoV estimation is more accurate for the current chunk compared to the future chunks and the weight for the quality variation is small, the above algorithm should work well. We prove that this is indeed the case in Theorem~\ref{thm:optimal}.  On the contrary, the second one (Algorithm~\ref{algo4}) tries to fetch the tiles of all the chunks of the same quality instead of fetching the tiles of the current chunk at the highest rate.  As expected, Algorithm~\ref{algo4} works well when the weight corresponding to the rate variation is high. %We then provide a simple heuristic to obtain the feasible solution from the optimal solution of the relaxed problem which also does not increase the stall time compared to the optimal one. The key idea behind the heuristic is that we first obtain the maximum possible permissible rates not exceeded by the optimal solution of the relaxed problem, then, we assign additional bandwidth within each chunk to download higher quality tiles which have higher probabilities to constitute the FoV.

%Although our first approach can maximize the expected QoE, it does not guarantee the bit-rate for the FoV with a high probability. If the FoV estimation has a lot of variances, the optimal solution which maximizes the expected QoE may render poor quality videos with a significant probability. \cite{feng,bao} also mentioned that the predicted head movement may not be accurate for a larger duration. Thus, as a second metric, we consider the QoE as the  bit-rate such that FoV will be at least that rate with probability $\alpha$ (Section~\ref{sec:robust}). The video service  provider wants to maximize the difference between the above rate and the weighted total stall time. We formulate the above problem as an optimization problem. %to maximize the above rate. %   the QoE is defined by the minimum rate  among the set of  tiles  which have very high probability to be the FoV. Hence, such an optimization problem will make sure that the FoV will be below that rate with a very low probability. %which constitute the event that the FoV will be within the set with a high probability.
%
% We propose an algorithm to solve the above problem.    We, also, provide a linear complexity heuristic algorithm which is optimal for a linear utility under the assumption that the FoV estimation is more accurate in the near future as compared to the distant future (Theorem~\ref{thm:optimal}). The above heuristic is similar to a greedy approach, where it will try to fetch the tiles  with a higher quality for a given chunk given that it does not exhaust the bandwidth and then will proceed to the subsequent chunks and so on. %We show that such a simple heuristic is optimal for a linear utility under the assumption that the FoV estimation is more accurate in the near future. We also propose another heuristic where in contrast to the above heuristic, it will fetch a higher quality tiles of a chunk if the similar quality tiles of other chunk can be downloaded within the estimated available bandwidth. We show that such a heuristic also provides a solution which is within the constant ratio of the optimal one, if the utilities do not increase much across the qualities.

%\fengout{We provide online version of the algorithm based on a sliding window type protocol. In the protocol, the decision of bit-rates at which tiles will be fetched is taken in an online fashion by optimizing over the limited time horizon. The uncertain head-movement, and the bandwidth prediction error are also considered.}
We use real users' head movement traces to evaluate our proposed algorithms. We use real time traces of the head-movement and the cellular bandwidth. 
%
Using the traces of the head positions of 40 users, we compute the empirical distribution of the FoV. We then apply our algorithm to the traces of 10 users.  The empirical results show that our proposed algorithms significantly outperform the baseline algorithms by at least in 30\% in the QoE metric. The baseline algorithms are considered to be the one which fetches all the tiles rather prioritizing those tiles which have higher chances to be viewed. We show that the average rate with which users will watch the video is almost 50\% higher than the baseline algorithms. Our empirical result also shows that our proposed algorithm outperforms the baseline algorithms by at least 60\%  in presence of higher bandwidth uncertainty. %  \feng{[[mention more results]].} %We consider two types of baseline algorithms, the {\em first} algorithm downloads the entire chunk in the same quality. The second one is a greedy type of algorithm and similar to the ones proposed in \cite{bao,feng}. This algorithm only fetches the tiles which have the highest probability to be part of the FoV.  In both of these baseline algorithms, we assume that if the bandwidth permits they will first try to fetch the current chunks at  higher qualities rather the subsequent chunks. We show that the QoE is greatly enhanced using our proposed algorithms compared to the above baseline algorithms. As our algorithm achieves at least 20\% higher QoE compared to the baseline algorithms. We also show that our algorithm provides 20\% higher average bit-rate within the FoV. Our algorithm significantly outperforms the baseline algorithms when the uncertainty regarding the bandwidth and the FoV prediction increase.

To summarize, our main contributions are as follows.

\begin{itemize}[leftmargin=*]

\item To the best of our knowledge, we propose the first principled algorithm that employs the formal method of stochastic optimization for streaming 360-degree videos. 
    It can directly work with crowd-sourced viewing statistics to make judicious decisions of prefetching tiles.
    Our approach explicitly takes into account the probabilistic nature of viewers' head movement randomness when watching 360-degree videos. 

%\fengout{To the best of our knowledge, this is the first work for 360-degree video streaming which formulates the QoE as the rate at which the user will see the video with probability $\alpha$ considering the statistics of the bandwidth estimation as well as the  distribution of the FoV.} %This is the first attempt to characterize the optimal strategy to maximize the QoE. %Note that similar metrics are already proposed in the communication channel (outage capacity \cite{tse2005,robust}), electricity market (robust optimization \cite{tsg_chen}), and cloud storage (tail latency \cite{infocom}).  The detailed formulation considers the statistics of the bandwidth estimation as well as the the distribution of the FoV.

\item The above QoE maximization problem is difficult to solve due to its non-convex nature. We propose efficient methods to solve it while achieving a bounded optimality gap (in terms of the QoE) that is independent of the number of chunks. We also design the online versions of the algorithm that dynamically adjust to the fluctuating bandwidth and uncertain head movement at runtime.

%However, there is no known polynomial time method to solve the discrete optimization problem. We, first, formulate a relaxed version of the problem by relaxing the integer discrete set. We propose an algorithm (Algorithm \textbf{360-ROBUST}) which yields a feasible solution from the optimal solution of the relaxed problem. We show that the optimality gap is independent of number of frames.
%\item We also provide an polynomial time algorithm to find feasible solution, and show that it is {\em optimal} under the scenario where the FoV prediction is more accurate in the near future rather than the distant future. We provide a polynomial time algorithm which minimizes the rate switch among two consecutive frames.
%\item We provi We provided a polynomial time algorithm to find a feasible solution. In fact, we show that the polynomial time algorithm is optimal under some assumptions which can be frequently observed in practice.

\item We evaluate our algorithms using real time traces. Using real users' head movement traces and real cellular bandwidth traces, we show using our emulation testbed that our proposed algorithms can achieve significantly higher QoE , higher average streaming rate compared to the baseline algorithms.
\end{itemize}



%\begin{itemize}[leftmargin=*]
%\item We formulate a QoE metric where we maximize the guaranteed rate that can be achieved with probability $\alpha$ while minimizing the stall time and the quality variation across the chunks.
%\item We formulate the optimization problem where the video service provider maximizes the above QoE metric.
%\item We provide low-complexity algorithms for  the proposed QoE metric. Each algorithm is suitable depending on the weight corresponding to the rate variation across the chunks.
%\item We use the real-time traces for the bandwidth and the FoV. Using our estimation approach for the real-time traces, we show that our proposed algorithms can achieve significantly higher QoE (at least in 30\% better) given the same bandwidth compared to the baseline algorithms.
%\end{itemize}

%\vspace{-.1in}
%\section{Related Literature}Recently, novel encoding schemes for 360-degree video streaming have been proposed \cite{Hosseini1,D'Acunto,occulus}. However, the above papers did not study the optimality of video streaming algorithms in terms of maximizing the perceived QoE  over the limited bandwidth.
%
%The authors of  \cite{yin,jiang} proposed algorithms for online video streaming under limited bandwidth which maximizes the QoE. However, these papers did not consider the {\em 360-degree videos}. The 360-degree videos pose unique challenges and thus require new metric for the QoE. For example,  in the 360-degree video, each chunk consists of several tiles. Hence, a video streaming algorithm now needs to find the rate at which each tile of a chunk has to be downloaded. In contrast, the above papers only need to find the rate at which a chunk has to be downloaded. In the 360-degree video, the FoV depends on the tiles of a chunk a user is viewing, the user may not view all the tiles, or in a viewing some tiles may be of different qualities which can impact the QoE. Hence, a new QoE metric is required for the 360-degree videos depending on the FoV.
\section{Related Literature}
 \cite{Xiao:2017,Xie:2017,Corbillon:2017} recently formulated mathematical models of QoE and proposed heuristic based algorithms. Heuristic based algorithms for 360-degree video streaming have been proposed   \cite{hosseini, Petrangeli}.   \cite{feng, bao} proposed an algorithm for streaming of tile-based 360-degree video streaming.  In the above papers  authors considered the short term prediction of the head movement and fetched tiles only along the predicted FoV. However, if the prediction is incorrect, a larger stall duration is incurred since the algorithm has to go back to fetch the chunks where prediction went wrong.  The head movement can only be known online and for a shorter time period, thus, the future videos can not be downloaded which can lead to a larger stall time when the bandwidth may be poor. Thus, we assume that each tile is fetched at least at the lowest quality so as not to stop to go back to fetch the chunks as that would also make the predictions very inaccurate.  Since the user likely wants to see the FoV in the same rate, the minimum rate in FoV determines the quality. Thus, this is the first work that considers robust optimization with the FoV and bandwidth prediction errors.   Further, there is no optimality guarantee of the  proposed heuristic algorithms in the prior works. We have characterized the optimality gap of our proposed algorithm.  The above papers also did not consider the quality variation across the chunks in the QoE metric.


  %We have also shown that our algorithm is in fact optimal when the user's perceived quality varies linearly with the streaming bit-rate.

 %In the above papers  authors considered the short term prediction of the head movement and fetched tiles only along the predicted FoV. However, the above papers did not consider the stall time in the QoE metric. The head movement can only be known online and for a shorter time period, thus, the future videos can not be downloaded which can lead to a larger stall time when the bandwidth may be poor. We have considered the stall time in the QoE metric and also the uncertainty of the bandwidth. Further, there is no optimality guarantee of the proposed heuristic algorithms. We have characterized the optimality gap of our proposed algorithms. We have also shown that our algorithm is in fact optimal when the user's perceived quality varies linearly with the streaming bit-rate. These papers proposed sending only those tiles which are part of the FoV. However, when the user changes his view, then he has to wait a certain amount of time for new tiles to be downloaded. Further, the above papers did not consider the robust QoE metric which we considered. Determination of the QoE metric for the tile based 360-degree video streaming based on the FoV, and the likelihood of a FoV being watched.  Recently, \cite{feng,bao} proposed FoV prediction based algorithms for the 360-degree video streaming. These papers estimate the FoV in the future  and fetch the tiles within that FoV. However, these papers did not provide any QoE metric for the 360-degree videos. Thus, there is no optimality guarantee for the heuristic. Second, the authors considered a sliding window protocol type protocol, where they predicted the FoV for a short time in the future and fetched the tiles in the predicted FoV. However, if there is an error in estimation, or the user views in some other areas, then there will be stall as the algorithm does not fetch anything outside the FoV. Third, these papers did not consider the quality variation across the chunks as a QoE. Finally, the algorithms provided in \cite{feng,bao} did not consider the download rates for future chunks. Thus, if the future bandwidth is limited, the user may observe poor quality video in the future.

%The closest to our work is our previous work \cite{previous}. \cite{previous} did not consider the rate variation across the chunks in the QoE metric. In contrast, we consider the quality variation of the FoV across the chunks. Thus, in contrast to \cite{previous}, we need to consider qualities for past chunks while downloading a future chunk. Thus, we need different algorithms for optimizing the overall QoE metric. Further, \cite{previous} does not consider the specific outage metric that we have in this paper. The proposed metric in this paper is practically important since having good quality in 95th percentile is sometimes more important than the mean. Such metrics have been considered in other areas, like communication channel (outage capacity \cite{tse2005}, \cite{robust}), electricity market (robust optimization \cite{tsg_chen}), and cloud storage (tail latency \cite{infocom}), while  it is new in 360-degree video streaming.  To the best of our knowledge, this is the first work which formulates the QoE as the minimum rate at which the user will see the video with probability $\alpha$ (or 100$\alpha$-th percentile rate). This is the first attempt to characterize the optimal strategy to maximize this QoE. The detailed formulation considers the statistics of the bandwidth estimation as well as the the distribution of the FoV. The QoE maximization problem turns out to be a discrete stochastic optimization problem. However, there is no known polynomial time method to solve the discrete optimization problem.  We provided a polynomial time algorithm to find a feasible solution. In fact, we show that the polynomial time algorithm is optimal under some assumptions which can be frequently observed in practice.


% Heuristic based algorithms for 360-degree video streaming have been proposed \cite{hosseini, ganainy}. These papers proposed sending only those tiles which are part of the FoV. However, when the user changes her view,  she has to wait a certain amount of time for new tiles to be downloaded.  Recently, \cite{feng,bao} proposed FoV prediction based algorithms for the 360-degree video streaming. These papers estimate the FoV in the future  and fetch the tiles within that FoV. However, these papers did not provide any QoE metric for the 360-degree videos. Thus, there is no optimality guarantee. Second, the authors considered a sliding window protocol, where they predicted the FoV for a short time in the future and fetched the tiles in the predicted FoV. However, if there is an error in estimation, or the user views in some other areas, there will be stall as the algorithm does not fetch anything outside the FoV. Third, these papers did not consider the quality variation across the chunks as a QoE. Finally, the algorithms provided in \cite{feng,bao} did not consider the download rates for future chunks. Thus, if the future bandwidth is limited, the user may observe poor quality video in the future.
%
%The closest to our work is  \cite{previous}, where  a QoE metric for the 360-degree video streaming is formulated. However, \cite{previous} did not consider the rate variation across the chunks in the QoE metric. In contrast, we consider the quality variation of the FoV across the chunks. Thus, in  contrast to \cite{previous}, we  need to consider qualities for past chunks while downloading a future chunk. Thus, we need different algorithms for optimizing the overall QoE metric. %  We consider both the distribution of the FoV estimation and the bandwidth. We provide low-complexity algorithms which maximize the above QoE metrics.

%The rest of the paper is organized as follows. Section \ref{sec:system} describes the system model and Section \ref{sec:robust} formulates the optimization problem. We further give equivalent problem statement and its convex relaxation in Section \ref{sec:robust}.  Low-complexity algorithms are provided in Section~\ref{sec:result}, which have been shown to  achieve significantly higher QoE compared to the baseline algorithms on trace-driven bandwidth and FoV profiles in Section~\ref{sec:simulation}. Section \ref{sec:add_sim} further considers the impact of larger variance of head movement  predictions. Finally, Section \ref{sec_concl} concludes the paper.


==> sims_mm.tex <==
\section{Trace-Driven Emulation Results}\label{sec:simulation}
%We, now, evaluate the strengths of our proposed algorithms in a simulated setting.
%\vspace{-.1in}

In this section, we empirically evaluate the performance of our algorithm based on the trace based emulation. We, first, explain how the bandwidth and FoV traces are collected and used to estimate in online manner. Subsequently, we explain our emulation set up. Finally, we compare our algorithms compared to two baseline algorithms.  %\feng{[[Better to have a pilot paragraph talking about the high-level approach for evaluation. Highlight it's emulation instead of simulation.]]}

\subsection{Bandwidth and FoV Traces }

\textbf{Bandwidth Traces}:  For bandwidth traces, we used a dataset from \cite{trace1}, which consists of continuous 1ms measurement of video streaming throughput of a moving device.  We use 40 traces which are at least 240 seconds long.
%\feng{[[The traces are for 3G. Can we use some newer traces such as this one: http://users.ugent.be/~jvdrhoof/dataset-4g/]]}

\textbf{FoV traces}: For FoV traces, we use a setting similar to the one described in \cite{feng}. Specifically, the trace consists of the head movement data of 50 users across the university.
Each user wears a Google Cardboard viewer \cite{cardboard} with
a Samsung Galaxy S5 smartphone placed into the back of
it. The smartphone plays four short YouTube 360 videos
(duration from 1min 40 sec to 3 min 26sec) of different genres. Meanwhile,
a head tracker app runs in the background and sends
the raw, yaw, pitch, and roll readings to a nearby laptop using
UDP over WiFi (latency less than 1ms). During the playback, the users can view at any
direction by freely moving their heads. We first compute the empirical distribution of the user's head movements by considering the data of 40  users. We then use the computed  empirical distribution as the distribution of the FoV for the remaining 10 users to construct the set $\mathcal{A}_{\alpha,k}$ for all $k$. % for the computing the optimal video quality for the sixth user using the algorithms that we describe.

    %In Section~\ref{sec:add_sim}, we will consider the impact of the FoV variance on the QoE attained by our proposed algorithms.  %At the $c$-th frame, we consider $\alpha$ as $\alpha+5*(k-c+1)/120$. %If the Note that the future prediction will be more erroneous, hence, the has higher cardinalities for future chunks rather than the current ones.

% In our simulation, the predicted bandwidth is computed by multiplying the actual value in the bandwidth trace by $1+e$ where $e$ is uniformly drawn from $[-p,p]$ where $0\leq p< 1$. Higher $p$ indicates higher variability. %We study the impact o$p$.
%\vspace{-0.1in}
%\subsection{Testbed Setup}
%In order to emulate the proposed approach, we  spatially segment the 360 video content into smaller
%portions called tiles. 

We take a 4 minute video, with a chunk duration of 2 seconds. The total number of chunks ($K$) is $120$.  The tile configuration for each chunk is considered to be $4\times 8$; each chunk consists of 32 tiles.   We considered an equi-rectangular projected video chunks. %\feng{[[What is a segment? Pay attention to the terms you use.]]}
Equi-rectangular projection is the most popular one because of its simplicity, and is also used by YouTube.The FoV is considered to be  120 degrees in the horizontal direction and 120 degree in the vertical direction \cite{feng}.% Since the FoV is considered to be the center of the video frame, in our case the FoV consists of a rectangle of $2\times 3$ tiles. The  \feng{[[Again, the FoV and its covered tiles may change depending on the viewing direction.]]}

The different tiles are encoded independently in different rates such that each chunk's rate is $x$ Mbps. We consider that the encoded rates belong to  $ \{8,16,24,32\}$. Since there are 32 tiles, each tile's average rate is $x/32$ Mbps which belongs to the  $\{0.25, 0.5, 0.75 ,1\}$. We transmit the video from the server, which is streaming to the client. 
%The video server
%runs on a Dell Power Edge R420 with a 6-core Intel E5-
%2620v3 CPU, 12 GB of RAM, and Ubuntu Server 16.0 LTS
%OS. The client is a Macbook Pro with 2.3GHz dual-core Intel Core i5, and 8GB memory. The server and client communicate with
%each other using the default TCP
%variant, TCP CUBIC \cite{ha2008cubic}. The client runs the bandwidth and FoV prediction to determine the qualities of the different tiles for the next chunk. This decision is sent to the server, and the server transmits the chunk with the tiles encoded at the requested quality levels. The emulation ends when
%all chunks are received. We record the received time of the chunk, and the
%quality  for each tile of the chunk.
%%
%To introduce bandwidth variations into the emulated experiments, we adopt
%Dummynet \cite{rizzo1997dummynet} running on the client side, thus the incoming
%rates of the TCP packets from the server  will be throttled according to the bandwidth trace used. Further, given the received qualities, the desired quality metrics are computed on the test FoV traces.

%the test FoV traces are used to compute the desired quality metrics. \feng{[[I don't understand the last sentence.]]}


In order to make the decision for the chunk quality, we employ the online algorithm that we have introduced in Section 4.3. %\feng{[[Refer to it using the section number.]]}
%
We run the online algorithm after the completion of the download of the each chunk for $W$ chunks ahead. Recall that $W$ is the size of the sliding window. Though our algorithm can update $W$ independently for each user, we fix  $W$  at the same value for each user. Unless explicitly mentioned, we assume that $W=5$. %We show the impact of the size of $W$. Except in Fig.~\ref{fig:window}, $W$ is set at $5$, as it obtains the optimal value when $W=5$.
  The utility function is assumed to be linear. Without loss of generality, we consider $U(x)=x$.   Recall from (\ref{eq:robust}) that $\lambda$ is the weight corresponding to the stall time. We assume $\lambda=100$, {\it i.e.}, we give more preference to minimize the stall time.  We set $\alpha$ as $0.95$, $x_k$ as $0.6$. %{\bf Arnob, Explain $\beta$, $W$, parameters of harmonic mean - how much past used, any dynamic window size policy used, etc. }
%\feng{[[Remind readers what $\alpha$ and $x_k$ are. Justify your parameter selection.]]}


\subsection{ Baseline Algorithms}
 We compare the online version of our proposed algorithm 360-ROBUST  with the following baseline algorithms (BA1 and BA2). %Note that since the utility is linear and the $|\mathcal{A}_{\alpha,k}|$ is the same for all $k$, hence by Theorem~\ref{thm:optimal} Algorithm 3 is optimal for $\mathcal{P}_{\text{robust}}$. We, thus, evaluate  the strengths of our proposed  Algorithms 1 and 3. For Algorithm 3, we set $\alpha$ at $0.95$. For comparison, we consider two simple strategies. These are explained in the following:

\textbf{BA1}: The first baseline algorithm will try to fetch all the tiles at the same quality. Thus, the qualities will be the same across the tiles.
If there is excess bandwidth, BA1 will first set the rate at the minimum rate possible for all the chunks. The algorithm then starts to set the rate at the next higher level for the last chunk if the stall time does not increase. The algorithm then does the same for the second last chunk. If there is still an additional bandwidth, the algorithm again sets the rate of the last chunk at the next highest level and so on. % The algorithm then again the tiles of the next higher qualities of the last chunk rather than the current chunk. The algorithm will then try to download the tiles in the next higher qualities of the second last chunk and so on.
%\feng{[[You shouldn't say ``fetch the tiles of the next higher qualities'' -- this is not feasible unless SVC is used. Instead this is part of the rate adaptation algorithm internals. Describe it in that way.]]}
Thus, similar to our proposed algorithm, BA1 uses extra bandwidth to fetch the tiles at higher qualities starting from the last chunk and so on. However, Algorithm 360-ROBUST  fetches the tiles within the set $\mathcal{A}_{\alpha,k}$ at a higher rate whereas BA1 fetches all the tiles  within a chunk  at the same rate. In addition, Algorithm 360-ROBUST also assigns the rate by solving a convex relaxation problem.

\textbf{BA2}: The second baseline algorithm, in contrast to the first one, fetches all the tiles of the current chunk at the highest possible rate if the bandwidth permits. Thus, the algorithm sets the highest possible rate for the current chunk such that all the tiles in the chunk can be fetched within the play-back time. 

This is a simple {\em greedy-type} algorithm, and thus, it is used widely in practice \cite{facebook}.
Similar to BA1, BA2 also fetches all the tiles within a chunk at the same rate. %  \feng{the following is unclear: in your Baseline algorithm, when you have extra BW, do you fetch the next chunk's tiles at a lower layer, or the current chunk's tiles at a higher layer?}


%This algorithm is This algorithm is proposed by \cite{feng}. The algorithm only fetches those tiles which have the highest probability to be the part of FoV. Again similar to the {\bf Baseline} algorithm it fetches the higher quality tiles of the current chunk first if there is an extra bandwidth before it fetches the tiles of the next chunk.  Though in this algorithm only a few tiles are required to be downloaded, if the prediction is not accurate, the viewer can see black spots even though it can save a lot of bandwidth. %\feng{This greedy algorithm is also not very clear. Need to provide more details of how it performs rate adaptation.}

We study the strength of our proposed algorithm Algorithm~360-ROBUST with respect to the two baseline algorithms. We evaluate the algorithms' achievable QoE (\ref{eq:robust}), the distributions of the bitrates in the FoV, and the impact of the window size $W$ on the overall QoE metrics by taking the average over 10 users. %We vary the identities of the 10 users and plot the worst case average result.  We also investigate the impact on the stall time, the bandwidth prediction error, and the FoV estimation error on the performance of our proposed algorithm. 

\vspace{-.1in}
\subsection{Results and Discussion}
\begin{figure}
	\vspace{-.1in}
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=.95\textwidth]{fov.pdf}
%\vspace{-0.2in}
%\caption{The tile based segmentation and the rectangular $2\times 3$ tiles is FoV with probability $\beta$.}
%\label{fig:fov}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.35\textwidth}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=0in 0.2in 0.5in 0in, clip, width=\textwidth]{qoevsalpha_mm.eps}
%\vspace{-0.2in}
\caption{ The variation of QoE with $\eta$.}
\label{fig:eta}
\end{minipage}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.35\textwidth}
%\includegraphics[width=.95\textwidth,height=1.6in]{qoevsbeta.eps}
%\vspace{-0.2in}
%\caption{The variation of QoE with $\beta$ for $\eta=1$.}
%\label{fig:beta}
%\vspace{-0.2in}
%\end{minipage}
%\vspace{-.1in}
%\end{figure}
%
%\begin{figure}
%\begin{minipage}{0.32\textwidth}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=0in 0.2in 0.5in 0in, clip,width=\textwidth]{rate_distr_mm.eps}
\vspace{-0.3in}
\caption{Rate distribution of the minimum rates among the tiles within set $\mathcal{A}_{\alpha,k}$ (or, $\gamma_k$) for $\eta=1$.]}
\label{fig:rate}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=.1in 0in 0.6in 0.3in, clip,width=\textwidth]{qoevsW.eps}
\caption{{The variation of QoE with the window size $W$ with $\eta=1$.}
%\feng{[[Y Axis label is not fully shown. Y should begin with 0]]}
}
\label{fig:window}
\end{minipage}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.32\textwidth}
%\includegraphics[width=.95\textwidth,height=1.6in]{quality_var.eps}
%\vspace{-0.2in}
%\caption{Total rate variation across the subsequent chunks (cf. (\ref{eq:diff})) as a function of $\beta$ for $\eta=1$.}
%\label{fig:quality}
%\vspace{-0.2in}
%\end{minipage}\hfill
%\begin{minipage}{0.32\textwidth}
%\includegraphics[width=.95\textwidth,height=1.7in]{stallvsbeta_stable.eps}
%\vspace{-0.2in}
%\caption{Variation of the total stall time with $\beta$.}
%\label{fig:stall}
\vspace{-0.2in}
%\end{minipage}
\end{figure}

%\feng{[[The biggest issue with evaluations is it's too short and simple. Expand the results section to at least 1.5 full pages (the methodology part is kinda verbose and can be further shortened). There are many other results that you can and should generate: the impact of FoV prediction, the impact of bandwidth prediction, the variation cross the users (try different sets of the 10 users), computation overhead, etc.]]}

 \subsubsection{Effect of $\eta$}
Recall from (\ref{eq:robust}) that $\eta$ is the weight corresponding to the quality variation across the chunks. Fig.~\ref{fig:eta} shows that as $\eta$ increases, the QoE decreases as is apparent from (\ref{eq:robust}). Since Algorithm 360-ROBUST is obtained from the optimal solution of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$, the performance of Algorithm 360-ROBUST would have been optimal if the number of quantization levels would have been large.

Note that the QoEs attained by the baseline algorithms are at least 30\% lower QoE compared to the our proposed algorithms.  Also note that BA2 is a greedy algorithm which tries to fetch the highest quality tiles for the current chunk. Hence, there will be more quality variation between subsequent chunks. Thus, the QoE attained by BA2 is the lowest. % the quality variation is smaller which gives higher QoE compared to BA2 when $\eta$ is high.

%\feng{[[It's unclear what the tradeoff is. I strongly recommend show different components of the QoE metrics separately (rate, stall, quality swtich) in addition to the current results.]]}

%\vspace{-.12in}

 \subsubsection{Distribution of the rates}
In Fig.~\ref{fig:rate}, we plot the distribution of the rates $\gamma_k$.  Most number of tiles are fetched at two nearby rates $0.5$ and $0.75$ Mbps. Algorithm 360-ROBUST also fetches a lot of tiles in the highest quality specifically for the later chunks where there is enough bandwidth for chunks to be fetched.

%Very few tiles are fetched at the highest rate. In contrast, Algorithm~\ref{algo3} fetches more number of tiles at the highest rate compared to Algorithm~\ref{algo4}. There is a lot more variation across the rates for the solution attained by Algorithm~\ref{algo4}. Algorithm~\ref{algo2} fetches lower number of tiles at highest rate compared to Algorithm~\ref{algo3}, however a higher number of tiles at the highest rate compared to Algorithm~\ref{algo4}. Algorithm~\ref{algo2} provides a solution where there is less variation across the rates  compared to Algorithm~\ref{algo3}, but has more variation compared to Algorithm~\ref{algo4}.

The two baseline algorithms hardly fetch any tiles at the highest rate. They mostly fetch the tiles at the lowest two possible rates. This is because BA1 and BA2 both need to fetch all the tiles within a chunk at the same quality. Thus, the bandwidth may not be enough to fetch the tiles at a higher rate. However, our proposed algorithm only fetches the tiles within the set $\mathcal{A}_{\alpha,k}$ at a higher rate, hence, lower bandwidth is required to give the same guaranteed rate. BA1 tries to equalize the rate among the chunks, hence, the distribution is close to inform over the chunks compared to BA2.

Our proposed algorithm provides the rate within the FoV with 50\% higher compared to the baseline algorithms. Intuitively, this is because the baseline algorithms download all the tiles within the chunk at a higher rate rather than only downloading the tiles within the set $\mathcal{A}_{\alpha,k}$. 

\begin{figure}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=.1in 0in 0.6in 0.3in, clip,width=\textwidth]{qoevsW.eps}
\caption{{The variation of QoE with the window size $W$ with $\eta=1$.}
%\feng{[[Y Axis label is not fully shown. Y should begin with 0]]}
}
\label{fig:window}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=.1in 0in 0.6in 0.3in, clip,width=\textwidth]{run_time.eps}
\caption{Variation of Run-time of Algorithm 360-ROBUST with $W$}
\label{fig:run_time}
\end{minipage}
\vspace{-0.2in}
\end{figure}

\subsubsection{Effect of the Window Size}
 Fig.~\ref{fig:window} shows that as the window size increases, the QoE increases. However, the QoE decreases after a threshold. Intuitively, if $W$ is large, the algorithm 360-ROBUST may be conservative, and only use excess bandwidth for fetching tiles at a higher quality for the last few chunks. The FoV or bandwidth prediction may also be bad if $W$ is large, specifically, if there is a temporal correlation where the prediction is highly correlated over short time period. On the other hand, if $W$ is too small, the algorithm may become too greedy, leading to a higher quality variation  between the subsequent chunks. $W=5$ performs the best. Note that our proposed algorithm outperforms the baseline algorithms by almost 35\%. Note that since BA2 is a greedy one, the impact of the variation of $W$ is the least on BA2. 
 
Fig.~\ref{fig:run_time} shows the average run-times (over different bandwidth traces) with the window size for our proposed algorithm {360-ROBUST}. The run-time is calculated on 8GB-DDR3 RAM and 1.6GHz Intel Core i5 processor, using a C++ code. Fig~\ref{fig:run_time} shows that as the window size increases the run-time increases. This is because the decision space increases with $W$. %However, the rate of increment decreases with the increase in the window size.
 
 \begin{figure}
 \vspace{-0.1in}
 \begin{minipage}{0.23\textwidth}
 \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{band.eps}
\caption{The variation of QoE with the bandwidth prediction error ($e$)}
\label{fig:band}
 \end{minipage}
 \begin{minipage}{0.23 \textwidth}
  \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{guranteed_mm.eps}
\caption{The variation of the rate such that the quality degrades below that rate only with probability $0.05$ with FoV prediction error ($\beta$).}
\label{fig:fov}
 \end{minipage}
 \vspace{-0.2in}
 \end{figure}
% \begin{figure}
% \includegraphics[trim=0.3in 0in 0.6in, clip,width=0.24\textwidth]{band.eps}
% 
% \label{fig:band}
% \vspace{-0.2in}
% \end{figure}
 
 \subsubsection{Impact of Bandwidth prediction Error}
 In order to study the impact of the bandwidth prediction error we multiply the original bandwidth traces by a factor $(1+p)$ where $p$ is a randomly chosen from an uniform distribution $[-e,e]$. The impact of the variation of QoE with $e$ is shown in Fig.~\ref{fig:band}. As $e$ increases the QoE decreases as the uncertainty increases. However, the decrement is very small compared to the baseline algorithms. The greedy algorithm's performance is worse compared to BA1 since BA1 tries to use the extra bandwidth for retrieving chunks at a relatively higher quality for later chunks unlike the greedy one. 
 
\subsubsection{Impact of FoV prediction Error}
In order to show the robustness of the algorithms, we have used the traces of the users' head-position with probability $\beta$ and randomly select a FoV with probability $1-\beta$. We characterize the performance of the algorithms as $\beta$ increases.  
 Fig.~\ref{fig:fov} shows that as $\beta$ decreases the performance of our proposed algorithm 360-ROBUST degrades. However, the rate with which the FoV will be seen with probability $0.95$ is still higher compared to the baseline algorithms. Note that as $\beta$ increases, the FoV becomes random. Thus, the performance coincides with the baseline algorithms as the cardinality of the set $\mathcal{A}_{\alpha,k}$ increases. Since the baseline algorithm fetches every tile in the chunk at the same rate, thus, the 95 percentile rate is constant even though $\beta$ decreases. 

\begin{figure}
\vspace{-0.1in}
\includegraphics[width=0.25\textwidth]{stallvsw.eps}
\vspace{-0.1in}
\caption{Variation of the stall time with window size ($W$)}
\label{fig:stall}
\vspace{-0.3in}
\end{figure}
\subsubsection{Stall Time}
Fig.~\ref{fig:stall} shows that our proposed algorithm again out performs the baseline algorithms. Our analysis reveals that as window size ($W$) increases the stall time decreases.  Intuitively, when $W$ is small the algorithm is greedy, and thus wants to utilize the extra bandwidth to fetch tiles of the current chunk only. Hence, if the future bandwidth is poor it may lead to a stall. Since BA2 is  greedy algorithm, thus, its stall is the highest. Also note that BA1's stall time is still higher compared to our proposed algorithm. This is because BA1 sets the same rate to all the tiles of a current chunk. Thus, in our proposed algorithm we save extra bandwidth by fetching the tiles of the set $\mathcal{A}_{\alpha,k}$ compared to BA1 which may be used to reduce the stall time for future chunks in the event when the bandwidth is very small. 
%\subsubsection{Runtime analysis}
%Fig.~\ref{fig:run_time} shows the average run-times (over different bandwidth traces) of  the Algorithms~\ref{algo3} and \ref{algo4} as a function of the window-size (in number of chunks). The run-time is calculated on 8GB-DDR3 RAM and 1.6GHz Intel Core i5 processor, using a C++ code. Note that one of the motivations behind introducing Algorithms~\ref{algo3} and \ref{algo4} are their lower complexity. Fig.~\ref{fig:run_time} indeed confirms the above intuition. The computational time  of Algorithm~\ref{algo3} is 48.6 ms, whereas that of the Algorithm~\ref{algo4} is 24.6ms, when $W=15$ chunks. Fig~\ref{fig:run_time} shows that as the window size increases the run-time increases. This is because the cision space increases with $W$. However, the rate of increment decreases with the increase in the window size. Also note that Algorithm~\ref{algo4} is faster compared to Algorithm~\ref{algo3}.




==> sims_mobicom.tex <==
\section{Trace-Driven Simulation Results}\label{sec:simulation}
%We, now, evaluate the strengths of our proposed algorithms in a simulated setting.
%\vspace{-.1in}

In this section, we empirically evaluate the performance of our algorithm based on the trace based simulation. We, first, explain how the bandwidth and FoV traces are collected and used to estimate in online manner.  Finally, we compare our algorithms compared to two baseline algorithms.  %\feng{[[Better to have a pilot paragraph talking about the high-level approach for evaluation. Highlight it's emulation instead of simulation.]]}

\subsection{Bandwidth and FoV Traces }

\textbf{Bandwidth Traces}:  For bandwidth traces, we used a dataset from \cite{trace1}, which consists of continuous 1ms measurement of video streaming throughput of a moving device.  We use 40 traces which are at least 240 seconds long.
%\feng{[[The traces are for 3G. Can we use some newer traces such as this one: http://users.ugent.be/~jvdrhoof/dataset-4g/]]}

\textbf{FoV traces}: For FoV traces, we use a setting similar to the one described in \cite{feng}. Specifically, the trace consists of the head movement data of 50 users across the university.
Each user wears a Google Cardboard viewer \cite{cardboard} with
a Samsung Galaxy S5 smartphone placed into the back of
it. The smartphone plays four short YouTube 360 videos
(duration from 1min 40 sec to 3 min 26sec) of different genres. Meanwhile,
a head tracker app runs in the background and sends
the raw, yaw, pitch, and roll readings to a nearby laptop using
UDP over WiFi (latency less than 1ms). During the playback, the users can view at any
direction by freely moving their heads. We first compute the empirical distribution of the user's head movements by considering the data of 40  users. We then use the computed  empirical distribution as the distribution of the FoV for the remaining 10 users to construct the set $\mathcal{A}_{\alpha,k}$ for all $k$. % for the computing the optimal video quality for the sixth user using the algorithms that we describe.

    %In Section~\ref{sec:add_sim}, we will consider the impact of the FoV variance on the QoE attained by our proposed algorithms.  %At the $c$-th frame, we consider $\alpha$ as $\alpha+5*(k-c+1)/120$. %If the Note that the future prediction will be more erroneous, hence, the has higher cardinalities for future chunks rather than the current ones.

% In our simulation, the predicted bandwidth is computed by multiplying the actual value in the bandwidth trace by $1+e$ where $e$ is uniformly drawn from $[-p,p]$ where $0\leq p< 1$. Higher $p$ indicates higher variability. %We study the impact o$p$.
%\vspace{-0.1in}
%\subsection{Testbed Setup}
%In order to emulate the proposed approach, we  spatially segment the 360 video content into smaller
%portions called tiles. 

We choose one of the videos with duration of 3 minutes used to compute the empirical distribution.  The chunk duration is assumed to be $2$ seconds. The total number of chunks ($K$) is $90$.  The tile configuration for each chunk is considered to be $4\times 8$; each chunk consists of 32 tiles.   We considered an equi-rectangular projected video chunks. %\feng{[[What is a segment? Pay attention to the terms you use.]]}
Equi-rectangular projection is the most popular one because of its simplicity, and is also used by YouTube.The FoV is considered to be  120 degrees in the horizontal direction and 120 degree in the vertical direction \cite{feng}.% Since the FoV is considered to be the center of the video frame, in our case the FoV consists of a rectangle of $2\times 3$ tiles. The  \feng{[[Again, the FoV and its covered tiles may change depending on the viewing direction.]]}

The different tiles are encoded independently in different rates such that each chunk's rate is $x$ Mbps. We consider that the encoded rates belong to  $ \{8,16,24,32\}$. Since there are 32 tiles, each tile's average rate is $x/32$ Mbps which belongs to the  $\{0.25, 0.5, 0.75 ,1\}$. We transmit the video from the server, which is streaming to the client. 
%The video server
%runs on a Dell Power Edge R420 with a 6-core Intel E5-
%2620v3 CPU, 12 GB of RAM, and Ubuntu Server 16.0 LTS
%OS. The client is a Macbook Pro with 2.3GHz dual-core Intel Core i5, and 8GB memory. The server and client communicate with
%each other using the default TCP
%variant, TCP CUBIC \cite{ha2008cubic}. The client runs the bandwidth and FoV prediction to determine the qualities of the different tiles for the next chunk. This decision is sent to the server, and the server transmits the chunk with the tiles encoded at the requested quality levels. The emulation ends when
%all chunks are received. We record the received time of the chunk, and the
%quality  for each tile of the chunk.
%%
%To introduce bandwidth variations into the emulated experiments, we adopt
%Dummynet \cite{rizzo1997dummynet} running on the client side, thus the incoming
%rates of the TCP packets from the server  will be throttled according to the bandwidth trace used. Further, given the received qualities, the desired quality metrics are computed on the test FoV traces.

%the test FoV traces are used to compute the desired quality metrics. \feng{[[I don't understand the last sentence.]]}


In order to make the decision for the chunk quality, we employ the online algorithm that we have introduced in Section 4.3. %\feng{[[Refer to it using the section number.]]}
%
We run the online algorithm after the completion of the download of the each chunk for $W$ chunks ahead. Recall that $W$ is the size of the sliding window. We assume that $W=5$. %We show the impact of the size of $W$. Except in Fig.~\ref{fig:window}, $W$ is set at $5$, as it obtains the optimal value when $W=5$.
  The utility function is assumed to be linear. Without loss of generality, we consider $U(x)=x$.   Recall from (\ref{eq:robust}) that $\lambda$ is the weight corresponding to the stall time. We assume $\lambda=100$, {\it i.e.}, we give more preference to minimize the stall time.  We set $\alpha$ as $0.95$, $x_k$ as $0.6$. %{\bf Arnob, Explain $\beta$, $W$, parameters of harmonic mean - how much past used, any dynamic window size policy used, etc. }
%\feng{[[Remind readers what $\alpha$ and $x_k$ are. Justify your parameter selection.]]}


\subsection{ Baseline Algorithms}
 We compare the online version of our proposed algorithm 360-ROBUST  with the following baseline algorithms (BA1 and BA2). %Note that since the utility is linear and the $|\mathcal{A}_{\alpha,k}|$ is the same for all $k$, hence by Theorem~\ref{thm:optimal} Algorithm 3 is optimal for $\mathcal{P}_{\text{robust}}$. We, thus, evaluate  the strengths of our proposed  Algorithms 1 and 3. For Algorithm 3, we set $\alpha$ at $0.95$. For comparison, we consider two simple strategies. These are explained in the following:

\textbf{BA1}: The first baseline algorithm will try to fetch all the tiles at the same quality. 
If there is excess bandwidth, BA1 will first set the rate at the minimum rate possible for all the chunks. The algorithm then starts to set the rate at the next higher level for the last chunk if the stall time does not increase. The algorithm then does the same for the second last chunk. If there is still an additional bandwidth, the algorithm again sets the rate of the last chunk at the next highest level and so on. % The algorithm then again the tiles of the next higher qualities of the last chunk rather than the current chunk. The algorithm will then try to download the tiles in the next higher qualities of the second last chunk and so on.
%\feng{[[You shouldn't say ``fetch the tiles of the next higher qualities'' -- this is not feasible unless SVC is used. Instead this is part of the rate adaptation algorithm internals. Describe it in that way.]]}
Thus, similar to our proposed algorithm, BA1 uses extra bandwidth to fetch the tiles at higher qualities starting from the last chunk and so on. However, Algorithm 360-ROBUST  fetches the tiles within the set $\mathcal{A}_{\alpha,k}$ at a higher rate whereas BA1 fetches all the tiles  within a chunk  at the same rate. In addition, Algorithm 360-ROBUST also assigns the rate by solving a convex relaxation problem.

\textbf{BA2}: The second baseline algorithm, in contrast to the first one, fetches all the tiles of the current chunk at the highest possible rate if the bandwidth permits. Thus, the algorithm sets the highest possible rate for the current chunk such that all the tiles in the chunk can be fetched within the play-back time. 

This is a simple {\em greedy-type} algorithm, and thus, it is used widely in practice \cite{facebook}.
Similar to BA1, BA2 also fetches all the tiles within a chunk at the same rate. %  \feng{the following is unclear: in your Baseline algorithm, when you have extra BW, do you fetch the next chunk's tiles at a lower layer, or the current chunk's tiles at a higher layer?}


%This algorithm is This algorithm is proposed by \cite{feng}. The algorithm only fetches those tiles which have the highest probability to be the part of FoV. Again similar to the {\bf Baseline} algorithm it fetches the higher quality tiles of the current chunk first if there is an extra bandwidth before it fetches the tiles of the next chunk.  Though in this algorithm only a few tiles are required to be downloaded, if the prediction is not accurate, the viewer can see black spots even though it can save a lot of bandwidth. %\feng{This greedy algorithm is also not very clear. Need to provide more details of how it performs rate adaptation.}

 We evaluate the algorithms' achievable QoE (\ref{eq:robust}), and the distributions of the bitrates in the FoV  on the overall QoE metrics by taking the average over 10 users. %We vary the identities of the 10 users and plot the worst case average result.  We also investigate the impact on the stall time, the bandwidth prediction error, and the FoV estimation error on the performance of our proposed algorithm. 

\vspace{-.1in}
\subsection{Results and Discussion}
\begin{figure}
	\vspace{-.1in}
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=.95\textwidth]{fov.pdf}
%\vspace{-0.2in}
%\caption{The tile based segmentation and the rectangular $2\times 3$ tiles is FoV with probability $\beta$.}
%\label{fig:fov}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.35\textwidth}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=0in 0.2in 0.5in 0in, clip, width=\textwidth]{qoevsalpha_mm.eps}
%\vspace{-0.2in}
\caption{ The variation of QoE with $\eta$.}
\label{fig:eta}
\end{minipage}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.35\textwidth}
%\includegraphics[width=.95\textwidth,height=1.6in]{qoevsbeta.eps}
%\vspace{-0.2in}
%\caption{The variation of QoE with $\beta$ for $\eta=1$.}
%\label{fig:beta}
%\vspace{-0.2in}
%\end{minipage}
%\vspace{-.1in}
%\end{figure}
%
%\begin{figure}
%\begin{minipage}{0.32\textwidth}
\begin{minipage}{0.23\textwidth}
\includegraphics[trim=0in 0.2in 0.5in 0in, clip,width=\textwidth]{rate_distr_mm.eps}
\vspace{-0.3in}
\caption{Rate distribution of the minimum rates among the tiles within set $\mathcal{A}_{\alpha,k}$ (or, $\gamma_k$) for $\eta=1$.]}
\label{fig:rate}
\end{minipage}
% \begin{minipage}{0.23\textwidth}
% \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{band.eps}
%\caption{The variation of QoE with the bandwidth prediction error ($e$)}
%\label{fig:band}
% \end{minipage}
% \begin{minipage}{0.23 \textwidth}
%  \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{guranteed_mm.eps}
%\caption{The variation of the rate such that the quality degrades below that rate only with probability $0.05$ with FoV prediction error ($\beta$).}
%\label{fig:fov}
% \end{minipage}
%\vspace{-0.2in}
%\end{minipage}
%\begin{minipage}{0.32\textwidth}
%\includegraphics[width=.95\textwidth,height=1.6in]{quality_var.eps}
%\vspace{-0.2in}
%\caption{Total rate variation across the subsequent chunks (cf. (\ref{eq:diff})) as a function of $\beta$ for $\eta=1$.}
%\label{fig:quality}
%\vspace{-0.2in}
%\end{minipage}\hfill
%\begin{minipage}{0.32\textwidth}
%\includegraphics[width=.95\textwidth,height=1.7in]{stallvsbeta_stable.eps}
%\vspace{-0.2in}
%\caption{Variation of the total stall time with $\beta$.}
%\label{fig:stall}
\vspace{-0.2in}
%\end{minipage}
\end{figure}

%\feng{[[The biggest issue with evaluations is it's too short and simple. Expand the results section to at least 1.5 full pages (the methodology part is kinda verbose and can be further shortened). There are many other results that you can and should generate: the impact of FoV prediction, the impact of bandwidth prediction, the variation cross the users (try different sets of the 10 users), computation overhead, etc.]]}

 \subsubsection{Effect of $\eta$}
Recall from (\ref{eq:robust}) that $\eta$ is the weight corresponding to the quality variation across the chunks. Fig.~\ref{fig:eta} shows that as $\eta$ increases, the QoE decreases as is apparent from (\ref{eq:robust}). Since Algorithm 360-ROBUST is obtained from the optimal solution of $\mathcal{P}^{\mathrm{relaxed}}_{\mathrm{eq}}$, the performance of Algorithm 360-ROBUST would have been optimal if the number of quantization levels would have been large.

Note that the QoEs attained by the baseline algorithms are at least 30\% lower QoE compared to the our proposed algorithms.  Also note that BA2 is a greedy algorithm which tries to fetch the highest quality tiles for the current chunk. Hence, there will be more quality variation between subsequent chunks. Thus, the QoE attained by BA2 is the lowest. % the quality variation is smaller which gives higher QoE compared to BA2 when $\eta$ is high.

%\feng{[[It's unclear what the tradeoff is. I strongly recommend show different components of the QoE metrics separately (rate, stall, quality swtich) in addition to the current results.]]}

%\vspace{-.12in}

 \subsubsection{Distribution of the rates}
In Fig.~\ref{fig:rate}, we plot the distribution of the rates $\gamma_k$.  Most number of tiles are fetched at two nearby rates $0.5$ and $0.75$ Mbps. Algorithm 360-ROBUST also fetches a lot of tiles in the highest quality specifically for the later chunks where there is enough bandwidth for chunks to be fetched.

%Very few tiles are fetched at the highest rate. In contrast, Algorithm~\ref{algo3} fetches more number of tiles at the highest rate compared to Algorithm~\ref{algo4}. There is a lot more variation across the rates for the solution attained by Algorithm~\ref{algo4}. Algorithm~\ref{algo2} fetches lower number of tiles at highest rate compared to Algorithm~\ref{algo3}, however a higher number of tiles at the highest rate compared to Algorithm~\ref{algo4}. Algorithm~\ref{algo2} provides a solution where there is less variation across the rates  compared to Algorithm~\ref{algo3}, but has more variation compared to Algorithm~\ref{algo4}.

The two baseline algorithms hardly fetch any tiles at the highest rate. They mostly fetch the tiles at the lowest two possible rates. This is because BA1 and BA2 both need to fetch all the tiles within a chunk at the same quality. Thus, the bandwidth may not be enough to fetch the tiles at a higher rate. However, our proposed algorithm only fetches the tiles within the set $\mathcal{A}_{\alpha,k}$ at a higher rate, hence, lower bandwidth is required to give the same guaranteed rate. BA1 tries to equalize the rate among the chunks, hence, the distribution is close to inform over the chunks compared to BA2.

Our proposed algorithm provides the rate within the FoV with 50\% higher compared to the baseline algorithms. Intuitively, this is because the baseline algorithms download all the tiles within the chunk at a higher rate rather than only downloading the tiles within the set $\mathcal{A}_{\alpha,k}$. 

%\begin{figure}
%\begin{minipage}{0.23\textwidth}
%\includegraphics[trim=.1in 0in 0.6in 0.3in, clip,width=\textwidth]{qoevsW.eps}
%\caption{{The variation of QoE with the window size $W$ with $\eta=1$.}
%%\feng{[[Y Axis label is not fully shown. Y should begin with 0]]}
%}
%\label{fig:window}
%\end{minipage}
%\begin{minipage}{0.23\textwidth}
%\includegraphics[trim=.1in 0in 0.6in 0.3in, clip,width=\textwidth]{run_time.eps}
%\caption{Variation of Run-time of Algorithm 360-ROBUST with $W$}
%\label{fig:run_time}
%\end{minipage}
%\vspace{-0.2in}
%\end{figure}

%\subsubsection{Effect of the Window Size}
% Fig.~\ref{fig:window} shows that as the window size increases, the QoE increases. However, the QoE decreases after a threshold. Intuitively, if $W$ is large, the algorithm 360-ROBUST may be conservative, and only use excess bandwidth for fetching tiles at a higher quality for the last few chunks. The FoV or bandwidth prediction may also be bad if $W$ is large, specifically, if there is a temporal correlation where the prediction is highly correlated over short time period. On the other hand, if $W$ is too small, the algorithm may become too greedy, leading to a higher quality variation  between the subsequent chunks. $W=5$ performs the best. Note that our proposed algorithm outperforms the baseline algorithms by almost 35\%. Note that since BA2 is a greedy one, the impact of the variation of $W$ is the least on BA2. 
% 
%Fig.~\ref{fig:run_time} shows the average run-times (over different bandwidth traces) with the window size for our proposed algorithm {360-ROBUST}. The run-time is calculated on 8GB-DDR3 RAM and 1.6GHz Intel Core i5 processor, using a C++ code. Fig~\ref{fig:run_time} shows that as the window size increases the run-time increases. This is because the decision space increases with $W$. %However, the rate of increment decreases with the increase in the window size.
% 
% \begin{figure}
% \vspace{-0.1in}
% \begin{minipage}{0.23\textwidth}
% \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{band.eps}
%\caption{The variation of QoE with the bandwidth prediction error ($e$)}
%\label{fig:band}
% \end{minipage}
% \begin{minipage}{0.23 \textwidth}
%  \includegraphics[trim=0.2in 0in 0.6in 0in, clip,width=\textwidth]{guranteed_mm.eps}
%\caption{The variation of the rate such that the quality degrades below that rate only with probability $0.05$ with FoV prediction error ($\beta$).}
%\label{fig:fov}
% \end{minipage}
% \vspace{-0.2in}
% \end{figure}
%% \begin{figure}
%% \includegraphics[trim=0.3in 0in 0.6in, clip,width=0.24\textwidth]{band.eps}
%% 
%% \label{fig:band}
%% \vspace{-0.2in}
%% \end{figure}
% 
% \subsubsection{Impact of Bandwidth prediction Error}
% In order to study the impact of the bandwidth prediction error we multiply the original bandwidth traces by a factor $(1+p)$ where $p$ is a randomly chosen from an uniform distribution $[-e,e]$. The impact of the variation of QoE with $e$ is shown in Fig.~\ref{fig:band}. As $e$ increases the QoE decreases as the uncertainty increases. However, the decrement is very small compared to the baseline algorithms. The greedy algorithm's performance is worse compared to BA1 since BA1 tries to use the extra bandwidth for retrieving chunks at a relatively higher quality for later chunks unlike the greedy one. 
 
%\subsubsection{Impact of FoV prediction Error}
%In order to study the impact of the FoV prediction error we use the exact trace of a user with probability $\beta$ and randomly select a FoV (uniformly among all choices), with probability $1-\beta$. Fig.~\ref{fig:fov} shows that as $\beta$ decreases the performance of our proposed algorithm 360-ROBUST degrades. However, the rate with which the FoV will be seen with probability $0.95$ is still higher compared to the baseline algorithms. Note that as $\beta$ increases, the FoV becomes random. Thus, the performance coincides with the baseline algorithms as the cardinality of the set $\mathcal{A}_{\alpha,k}$ increases. Since the baseline algorithm fetches every tile in the chunk at the same rate, thus, the 95 percentile rate is constant even though $\beta$ decreases. 
%
%\begin{figure}
%\vspace{-0.1in}
%\includegraphics[width=0.25\textwidth]{stallvsw.eps}
%\vspace{-0.1in}
%\caption{Variation of the stall time with window size ($W$)}
%\label{fig:stall}
%\vspace{-0.3in}
%\end{figure}
%\subsubsection{Stall Time}
%Fig.~\ref{fig:stall} shows that our proposed algorithm again out performs the baseline algorithms. Our analysis reveals that as window size ($W$) increases the stall time decreases.  Intuitively, when $W$ is small the algorithm is greedy, and thus wants to utilize the extra bandwidth to fetch tiles of the current chunk only. Hence, if the future bandwidth is poor it may lead to a stall. Since BA2 is  greedy algorithm, thus, its stall is the highest. Also note that BA1's stall time is still higher compared to our proposed algorithm. This is because BA1 sets the same rate to all the tiles of a current chunk. Thus, in our proposed algorithm we save extra bandwidth by fetching the tiles of the set $\mathcal{A}_{\alpha,k}$ compared to BA1 which may be used to reduce the stall time for future chunks in the event when the bandwidth is very small. 
%\subsubsection{Runtime analysis}
%Fig.~\ref{fig:run_time} shows the average run-times (over different bandwidth traces) of  the Algorithms~\ref{algo3} and \ref{algo4} as a function of the window-size (in number of chunks). The run-time is calculated on 8GB-DDR3 RAM and 1.6GHz Intel Core i5 processor, using a C++ code. Note that one of the motivations behind introducing Algorithms~\ref{algo3} and \ref{algo4} are their lower complexity. Fig.~\ref{fig:run_time} indeed confirms the above intuition. The computational time  of Algorithm~\ref{algo3} is 48.6 ms, whereas that of the Algorithm~\ref{algo4} is 24.6ms, when $W=15$ chunks. Fig~\ref{fig:run_time} shows that as the window size increases the run-time increases. This is because the cision space increases with $W$. However, the rate of increment decreases with the increase in the window size. Also note that Algorithm~\ref{algo4} is faster compared to Algorithm~\ref{algo3}.




==> system_mobicom.tex <==
\section{System Model}\label{sec:system}
Suppose that the video consists of  $K$ chunks.  Each chunk corresponds to certain temporal segment of the video. Each chunk is of duration $L$ seconds. Hence, the total duration of the video is $KL$ seconds. We consider non-real time video streaming, {\it i.e.}, a video has been recorded previously and needs to be streamed to the users as per their requests. However, the algorithms we propose can be extended to the live TV streaming with a minor modification.
Each chunk $k=1,\ldots, K$ has $N$ tiles in total of the same duration\footnote{We do not assume any fixed shape and size of the FoV. However, the entire chunk has to be divided in different number of tiles. Our analysis will go through even if the number of tiles is different across the chunks. }. The tiles constitute sub-areas within a chunk.
A tile has the same duration as the chunk.  %\feng{Can we have a table that lists all notions?}

\textbf{Field of View}: A viewing area for chunk $k$ belongs to the set  $\mathcal{V}_k$ which is the set of sub-sets of $l$ tiles among all $N$ tiles. Thus, the field of view (FoV) $V_{f,k}\in \mathcal{V}_k$ consists of $l$ tiles of a chunk. The video player can choose to download tile $i\in \{1,\ldots, N\}$ of chunk $k$ at the rate $R_{i,k}$. Thus, $L\sum_{i}^{N}R_{i,k}$ is the size of the chunk $k$. %To illustrate the FoV, consider the following example, suppose the tile representation of the entire viewing area be $4\times 8$. If the FoV consider


Quality difference among the tiles within a FoV severely degrades the QoE. Thus, we assume that the video player adapts the rate of the video at the minimum rate among the tiles in the FoV  which are downloaded. Thus, even though the tiles are downloaded at different rates, it is displayed at the minimum rate among all the tiles within the FoV. %Thus, there is no quality difference among the tiles within the FoV which will increase the QoE.%\feng{[[Why are you adopting this assumption? Justify it. One possible justification is that it minimizes the quality differences among tiles, leading to better user QoE.]]}


% if the tile $i$ of chunk $k$ is downloaded at the rate $R_{i,k}$

\textbf{Encoding Scheme}: %We consider the scalable video coding (SVC) for encoding the video\cite{}. Although much newer than many existing encoding schemes, SVC has existed for a while: it received the final approval to be standardized as an amendment of the H.264/MPEG-4 AVC standard in 2007\cite{}. The basic idea of SVC is to encode a chunk into ordered layers: one base layer (Layer 0) with the lowest playable quality, and multiple enhancement layers (Layer i >0) that further improve the chunk quality based on layer i ? 1. When downloading a chunk, a player must download all layers from 0 to i before fetching layer i + 1.
We consider that each chunk is encoded in one of the predefined quality layers. Each layer corresponds to a bit-rate.
The bit-rate $R_{j}$ denotes the rate at the $j$-th layer. Thus, the tile $i$ within a chunk $k$ can be downloaded at rate  $R_{i,k}\in \{R_0,R_1,\ldots, R_{m}\}$ where $R_{m}>\ldots>R_1>R_0$. Hence, the set of possible rates is the same for each tile. 

Note that if the FoV coincides with the tiles where those tiles have been downloaded at zero rate, the user may see black spots. In order to avoid that  we assume that the video player has to download a tile at least at its minimum rate $R_0$. Thus, even if the FoV prediction is erroneous, the user will not watch any black spots. Note that in contrast, the most literature \cite{hosseini, ganainy, Graf, Petrangeli, LeFeuvre, feng, bao} considered to download tiles only within the predicted FoV. Thus, if the prediction is erroneous, the user will  see black spots. 
Our approach can work both with the Adaptive Video Coding (AVC) \cite{avc}  or Scalable Video Coding (SVC) \cite{svc}.
%\feng{Change ``DASH'' to AVC (Adaptive Video Encoding) since DASH can work with either AVC or SVC. Mention the key difference between AVC and SVC is that in AVC, each video chunk is stored into independent encoding versions while in SVC the encoding of one version may depend on that of another version.}
 %The main difference between AVC and SVC is that in AVC, each video chunk is stored into independent encoding versions while in SVC the encoding of one version may depend on that of another version. AVC is easy to implement and thus, it is the most popular one. However, SVC's unique encoding scheme has many advantages over the other state-of-the-art schemes.  For example,  if the chunk in AVC is not fully downloaded before its playback deadline, there will be a stall. However, this can be easily mitigated in the SVC: if a chunk can not be downloaded at layer $j+1$, it still can be played without any stall for layer up to $j$.
%We highlight the coding scheme that will be useful in each problem formulation or implementation of our proposed algorithms. %In the 360-degree videos, the FoV has to be estimated. However, if the actual view is different compared to the predicted FoV, the SVC can still play at the lowest possible rate if it is pre-fetched before. On top of this base layer, enhancement layers can be downloaded in the real time.  Also note that if there is a quality variation among different tiles within a FoV, using the SVC encoding scheme the video player can adjust to play at the minimum rate among the tiles which is not possible in the DASH. %The rate or quality with which the chunk $k$ is played depends on the quality of the tiles in a viewing area which has been downloaded. Hence, if the FoV is $V_{k}\in \mathcal{V}_k$, then the quality is $\min_{j\in V_{k}}R_{j,k}$. Even if the tiles within a FoV are downloaded at different rates, the video player can adjust to play at the minimum rate among the tiles.

 %as shown on the right side of Figure 1.As of today, SVC has not yet registered wide deployment in commercial video platforms likely due to itscomplexity and a lack of use cases. Also as expected, much less academic research has been conducted onSVC compared to DASH-style schemes.

% Hence,


\textbf{Download time and Bandwidth}: Different chunks of video are downloaded sequentially into a {\em playback buffer} which contains downloaded but as yet unwatched video. Let $B(t)\in [0,B_{max}]$ denote the buffer occupancy at time $t$, {\it i.e}., the play-time of the video left in the buffer at time $t$.  Chunk $k+1$ can be started to download once the chunk $k$ is downloaded. Once the chunk $k$ is downloaded, the video player waits a time $\zeta_k$ to start downloading the chunk $k
=1$. Specifically, $\zeta_k$ is positive only when the buffer is full, otherwise, it is $0$. Let $t_k$ be the start time of downloading the chunk $k$. We have:
\begin{align}\label{eq:tk}
t_{k+1}=t_{k}+\dfrac{L\sum_{i}R_{i,k}}{C_k}+\zeta_k,\quad t_0=0.
\end{align}
 where $C_k$ is the average bandwidth while downloading the chunk $k$, {\it i.e.}, in the interval $[t_k,t_{k+1}]$. We assume that $C_k$ can be estimated which we explain in detail in Section 5.2.
 %\footnote{\fengout{Our model also allows the scenario where the bandwidth can be estimated on any time scale. If the time-scale overlaps with the download time $[t_k,t_{k+1}]$ one can easily get the total time by computing the time in each interval the bandwidth is estimated.}} \fengout{Note that even though the duration of a video can be a few minutes, the duration of chunk is only a few seconds.}  %Note that in our algorithm the tiles which constitute the set $\mathcal{A}_k$ for chunk $k$,
% \fengout{We further note that the performed evaluations considers trace based bandwidth, where the harmonic mean prediction is used to estimate the future bandwidth. We do not need a perfect prediction of the bandwidth, only a statistics will be sufficient.
  % Even if the mean of the bandwidth can not be accurately predicted, we will make a conservative approximation for the bandwidth and assume that $C_k$ be the worst possible bandwidth (or, the $C_k$ be the number such that the bandwidth during time $[t_k,t_{k+1}]$ will be higher than $C_k$ with a high probability).} \feng{[[Talk about evaluation stuffs in the evaluation section, not here!]]}

%
% Since the VR applications are getting popular, users are most likely to watch it on wireless devices such as phones, and tablets. They are mostly mobile. The mobility can affect the stability of the connection. Hence, the bandwidth can vary significantly over the time. Even if the the user is static, the bandwidth can vary depending on how many users are using the channel and the channel gain at a specific time. The number of users, and the channel gain evolve randomly over time. Thus, it is expected that there will be randomness in the bandwidth. Hence, we need an efficient algorithm which considers both the uncertainty in the bandwidth as well the uncertainty in the FoV.
%

\textbf{Play time of a chunk}: The buffer occupancy evolves as new chunks are downloaded. When a chunk is downloaded the buffer occupancy increases by $L$ and when the chunk is played, it decreases by $L$. We denote the play-time of the $k$-th chunk as $\tilde{t}_k$, i.e., the $\tilde{t}_k$ is the time when the $k$-th chunk starts playing. If the chunk $k$ is not downloaded before its designated time $\tilde{t}_{k-1}+L$, it has to wait till chunk $k$ is downloaded. The time at which chunk $k$ is downloaded is given by $t_{k-1}+\dfrac{L\sum_{i}R_{i,k}}{C_k}$. %\fengout{Note that the $k$-th chunk can only start playing only when the k-th chunk is downloaded. Hence,} 

Hence, for chunk $k>1$, the play time is:
\begin{align}\label{b_k}
\tilde{t}_{k}=\max\left\{\tilde{t}_{k-1}+L,t_{k-1}+\dfrac{L\sum_{i}R_{i,k}}{C_k}\right\}, \quad \tilde{t}_1=t_{\mathrm{ini}}.
\end{align}
where $t_{\mathrm{ini}}$ is the initial start-up time or initial stall time. This is the time the first chunk starts playing. The initial start-up time is often considered to be constant.% \feng{[[give intuition of (2)]]}
%The buffer occupancy evolves as new chunk is downloaded. When a chunk is downloaded it is increased by $L$ and when the  chunk is played, it decreases. The evolution of the buffer occupancy is characterized in the following--
%\begin{align}\label{b_k}
%B_{k+1}=((B_k-\dfrac{d_k(\sum_{i=1}^{N_k}R_{i,k})}{C_k})^{+}+L-\alpha_k)^{+}.
%\end{align}

\textbf{Stall time}: Note that each chunk constitutes $L$-second worth of video content. Hence, if $\tilde{t}_{k}>(k-1)L+t_{\mathrm{ini}}$, then, there will be stall or re-buffering. Thus the total stall time is $(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})^{+}$.  Note from (\ref{b_k}) that $\tilde{t}_{K}\geq (K-1)L+t_{\mathrm{ini}}$.  Thus,
\begin{align}\label{stall}
(\tilde{t}_K-(K-1)L-t_{\mathrm{ini}})^{+}=\tilde{t}_K-(K-1)L-t_{\mathrm{ini}}.
\end{align}
 %If the FoV prediction is wrong, and tiles are not downloaded in FoV, there could be additional stalls. Also, this stall may make the entire FoV prediction incorrect. In order to avoid such stalls, we assume that each tile of every chunk is downloaded at the minimum rate.
%$\dfrac{d_k(\sum_{i=1}^{N_k}R_{i,k})}{C_k}>B_k$, the buffer becomes empty while still downloading the chunk $k$. Hence, there will be stall or re-buffering.

\textbf{Maximum Buffer Occupancy}: As mentioned before we assume that as soon as chunk $k$ is downloaded, the video player starts downloading the chunk $k+1$. Hence, $\zeta_k$ is $0$ when the buffer is not full. However one exception is that when the buffer is full, the player waits for the buffer occupancy level to decrease so that the next chunk can be downloaded.

Without loss of generality, we assume that the maximum buffer occupancy is a multiple of $L$. The buffer can store at most $B$ chunks. Hence, we must have
\begin{align}\label{eq:max_buffer}
t_{B+k}\geq \tilde{t}_k\quad k=1,\ldots, K-B.%\alpha_k=((B_k-\dfrac{d_k(\sum_{i=1}^{N_k}R_{i,k})}{C_k})^{+}+L-B_{max})^{+}.
\end{align}
$\zeta_k$ is adjusted in (\ref{eq:tk}) such that the above constraint is satisfied. Currently, the maximum buffer occupancy $B$ can be very high, and, therefore, the above constraint is almost always satisfied. % with $\zeta_k=0$ for all $k$. \feng{[[so what? how does this affect the algorithm design?]]}

\textbf{User's utility}:
The user obtains an utility $U(\cdot)$ depending on the rate at which the video is being played. For example, if the chunk is played at rate $R$, the user's utility is $U(R)$ which denotes the user's satisfaction for getting the chunk at rate $R$. $U(\cdot)$ is a strictly increasing function as the user strictly prefers a higher rate.
The play-back rate for a chunk in the FoV is governed by the lowest rate amongst the tiles within the FoV since the video is played at the lowest rate among all the tiles within the FoV.

We assume that
\begin{assumption}
$U(\cdot)$ is a concave strictly-increasing function.
\end{assumption}
%\vspace{-.1in}

The intuition behind the above assumption is that user's QoE increases very fast initially with the play back rate of the video, however, the user becomes more indifferent when the play back rate exceeds a certain threshold. 
This is a standard assumption as the user utilities are often assumed to be concave (e.g., smart grid \cite{low2}, quality of service for multimedia \cite{wang}). $U(x)=x^{\alpha}$ where $\alpha\leq 1$ is an example of a concave function.

